Improving DRAM Performance, Reliability, and Security by Rigorously Understanding Intrinsic DRAM Operation

DRAM is the primary technology used for main memory in modern systems. Unfortunately, as DRAM scales down to smaller technology nodes, it faces key challenges in both data integrity and latency, which strongly affect overall system reliability, security, and performance. To develop reliable, secure, and high-performance DRAM-based main memory for future systems, it is critical to rigorously characterize, analyze, and understand various aspects (e.g., reliability, retention, latency, RowHammer vulnerability) of existing DRAM chips and their architecture. The goal of this dissertation is to 1) develop techniques and infrastructures to enable such rigorous characterization, analysis, and understanding, and 2) enable new mechanisms to improve DRAM performance, reliability, and security based on the developed understanding. To this end, in this dissertation, we 1) design, implement, and prototype a new practical-to-use and flexible FPGA-based DRAM characterization infrastructure (called SoftMC), 2) use the DRAM characterization infrastructure to develop a new experimental methodology (called U-TRR) to uncover the operation of existing proprietary in-DRAM RowHammer protection mechanisms and craft new RowHammer access patterns to efficiently circumvent these RowHammer protection mechanisms, 3) propose a new DRAM architecture, called SelfManaging DRAM, for enabling autonomous and efficient in-DRAM maintenance operations that enable not only better performance, efficiency, and reliability but also faster and easier adoption of changes to DRAM chips, and 4) propose a versatile DRAM substrate, called the Copy-Row (CROW) substrate, that enables new mechanisms for improving DRAM performance, energy consumption, and reliability.

==> mainmatter/crow/0_abstract.tex <==
\begin{abstract}

    DRAM has been the dominant technology for architecting main memory for
    decades. Recent trends in multi-core system design and
    large-dataset applications have amplified the role of DRAM as a
    critical system bottleneck.  We propose Copy-Row DRAM (\mech), a
    flexible substrate that enables new mechanisms for improving DRAM
    performance\hh{, energy efficiency, and reliability}. We use \mip{the} \mech
    substrate to implement 1)~a low-cost in-DRAM caching mechanism that
    lowers DRAM activation latency to frequently-accessed rows by 38\% and
    2)~a \sgii{mechanism that avoids the use of} \mip{short}-retention-time rows to mitigate the
    performance and energy overhead of DRAM refresh operations. {\mech}'s
    flexibility \hh{allows} \hho{the implementation of} both mechanisms \hh{at the same
    time}. Our evaluations show that the two mechanisms synergistically
    improve system performance by \hhb{20.0\%} and reduce DRAM energy by \hha{22.3\%}
    for memory-intensive four-core workloads, while incurring
    \hho{0.48\% \hhs{extra area overhead in the DRAM chip}}
    and \SI{11.3}{\kibi\byte} storage overhead in the
    memory controller\hho{, \hhs{and consuming 1.6\% of DRAM storage
    capacity,} for one particular implementation}.

    % \todo{update other parts that related to the area overhead like in the
    % abstract}
\end{abstract}


==> mainmatter/crow/10_acknowledgments.tex <==
\vspace{-1mm}
\section*{Acknowledgments}

\sgii{We thank the anonymous reviewers for feedback. We thank the SAFARI
Research Group members for feedback and the stimulating intellectual
environment they provide. We acknowledge the generous \hha{gifts provided by}
our industrial partners: Alibaba, \hha{Facebook}, Google, Huawei, Intel,
Microsoft, and VMware. This research was supported in part by the Semiconductor
Research Corporation.}


==> mainmatter/crow/1_intro.tex <==
% !TEX root=../main.tex

%\vspace{-2mm}

\section{Introduction}
\label{crow_sec:intro}

DRAM has long been the \hhs{dominant} technology \hho{for} architecting main
memory systems due to the high capacity it offers at low cost.
%%DRAM-based memory architectures are hierarchically designed to provide
%%low access latency for memory accesses with good \hhm{spatio-temporal} locality.
%%
%%%
%%%However, recent trends in multi-core system design and applications
%%%show increasing demand for data and decreasing spatial locality in
%%%memory accesses \todo{is the statement about spatial locality true?}. 
%%%This results in long DRAM access latencies and a poor
%%%utilization of the maximum available DRAM bandwidth. 
%%%
%%\hhm{However, trends in multi-core system design and applications
%%negatively affect access locality, \hho{leading} to long DRAM access
%%latencies and poor DRAM bandwidth utilization~\cite{jevdjic2014unison,
%%lotfi2012scale, jevdjic2013stacked,
%%ferdman2012clearing, palit2016demystifying, kanev2015profiling}.}
%%
%%
%%\hh{Thus},
%DRAM is a critical bottleneck for
%application performance \hhm{and important source of energy inefficiency in
%modern systems}~\cite{mutlu2015research}. To mitigate \hho{the
%performance, energy consumption, and reliability issues of DRAM},
%\hhm{several} works~\cite{liu2012raidr, hassan2016chargecache,
%choi2015multiple, kim-isca2012, lee-hpca2013, lee-hpca2015,
%chandrasekar2014exploiting, venkatesan2006retention, shin2014nuat,
%son2013reducing, lee2016reducing, chang2014improving,
%mukundan2013understanding, chang2016low} identify two major challenges to
%address: 1)~high DRAM access latency and 2)~high DRAM refresh overhead. 
%%Prior \hh{works
%%propose} techniques to reduce both~\cite{liu2012raidr,
%%hassan2016chargecache, choi2015multiple, kim-isca2012, lee-hpca2013,
%%lee-hpca2015, chandrasekar2014exploiting, venkatesan2006retention,
%%shin2014nuat, son2013reducing, lee2016reducing, chang2014improving,
%%mukundan2013understanding, chang2016low}.
%
\sg{As the memory demands of applications have been growing,
manufacturers have been scaling the DRAM process technology to
keep pace.
Unfortunately, while the density of the DRAM chips has been increasing
as a result of scaling, DRAM faces three critical challenges in
meeting application demands~\cite{mutlu2015research, mutlu2013memory}:
(1)~high access latencies and
(2)~high refresh overheads, both of which \hha{degrade} system performance
and energy efficiency; and
(3)~increasing exposure to vulnerabilities, which \hhs{reduces} the
reliability of DRAM.}
% \hho{However, DRAM is a critical bottleneck for
% application performance and significant contributor to energy 
% consumption in modern systems~\cite{mutlu2015research}.}
% \hho{Although continued scaling of DRAM process technology
% improves device density, DRAM faces critical challenges that 
% negatively impact system performance, energy consumption, and reliability.}

\hho{First, \sg{the} high DRAM access latency is \sg{a} challenge to improving system
performance and energy \sg{efficiency.}}
While
DRAM capacity increased significantly over \sg{the last two}
decades~\cite{standard2007ddr3, standard2013ddr4, son2013reducing,
chang2016understanding, lee-hpca2013, lee-hpca2015}, DRAM access latency
decreased only slightly~\cite{lee-hpca2013, mutlu2015research,
chang2016understanding}.
%  as commodity DRAM is primarily optimized for
% low cost-per-bit.
%The first major challenge is high DRAM access latency. \hhm{DRAM latency
\hhm{\sg{The high DRAM access latency} significantly \hha{degrades} the performance of many
workloads~\cite{ferdman2012clearing, huang2014moby, gutierrez2011full,
zhu2015microarchitectural, hestness2014comparative}\sg{.
The \hhs{performance impact} is particularly large for applications} that 1)~have working sets
exceeding the cache capacity of the system, 2)~suffer from high instruction
and data cache miss rates, and 3)~have low memory-level parallelism.}  
\sg{While manufacturers} offer latency-optimized DRAM
modules~\cite{rldram, sato1998fast}, \sg{these} modules have
\hho{significantly} lower capacity and higher cost compared to commodity
DRAM~\cite{lee-hpca2013, chang2016low, kim-isca2012}. 
%Therefore, current
%latency-optimized DRAM modules are not suitable for the majority of modern
%workloads that operate on large volumes of data~\cite{jevdjic2014unison,
%lotfi2012scale, qureshi2007adaptive, qureshi2007line}. 
Thus, reducing the high DRAM access latency \emph{without trading off
capacity and cost} in commodity DRAM remains an important 
challenge\hha{~\cite{ghose.sigmetrics19, ghose.arxiv19, lee-hpca2013, mutlu2013memory}}.

\hho{Second, \sg{the high} DRAM refresh overhead \sg{is a challenge to improving}
system performance and energy consumption.}
%The second major challenge is the high \hhm{performance and energy}
%overhead of DRAM refresh. 
\sg{A DRAM cell stores data in a capacitor that leaks charge over time.
To maintain correctness, \emph{every} DRAM cell requires periodic
\sg{\emph{refresh} operations that restore the charge level in a cell.}} 
% to maintain data correctness. This refresh operation must be
% performed on \emph{every} DRAM cell. 
As \sg{the} DRAM cell size decreases with
process \sg{technology} scaling, 
\sg{newer DRAM devices contain more DRAM cells than older
DRAM devices~\cite{itrs}}.
% new generation DRAM devices accommodate more DRAM
% cells~\cite{itrs}. 
\hhm{As a result}, 
%although more cells provide higher capacity
\hhm{while DRAM capacity increases}, the performance and energy \hho{overheads} of the refresh
operations \hho{scale} unfavorably~\cite{chang2014improving, kang-memcon2014,
liu2012raidr}. 
%Due to process variation, DRAM cells do not have identical
%retention times. \hhm{Therefore, some} DRAM cells retain their data for intervals as
%short as \SI{64}{\milli\second} \hhm{while others for} many
%minutes \hhm{or longer}~\cite{liu2012raidr, chang2014improving, patel2017reach,
%liu2013experimental, mukundan2013understanding, nair2014refresh,
%qureshi-dsn2015, liu2012flikker, nair2013case, stuecheli2010elastic,
%jung2015omitting, isen2009eskimo}. 
%However, existing schemes refresh all
%DRAM cells uniformly at a fixed refresh interval and therefore 
\hho{In modern LPDDR4~\cite{micron-lpddr4} devices, the memory controller
refreshes} \emph{every} DRAM cell every \hho{\SI{32}{\milli\second}}.
Previous studies show that 1)~refresh operations incur large performance
\sg{overheads,} as DRAM cells \emph{cannot} be accessed \sg{when the cells
are being refreshed}~\cite{chang2014improving, liu2012raidr, mukundan2013understanding,
nair2014refresh}; and 2)~up to 50\% of \sg{the} total DRAM energy is consumed by the
refresh operations\sgii{~\cite{liu2012raidr, chang2014improving}}. 


\hho{Third, \sg{the increasing \hhs{vulnerability of} DRAM cells \hhs{to
various \mip{failure mechanisms} is} an
important challenge to maintaining DRAM reliability.
As the} process technology shrinks, DRAM cells \hhs{become smaller and} get closer to each
other, and \hhs{thus} become more susceptible to
\hhs{failures~\cite{mandelman2002challenges, mutlu2013memory,
redeker2002investigation, yaney1987meta, konishi1989analysis, liu2012raidr,
liu2013experimental}}.
%  that negatively impacts DRAM realiability.
\hhs{A tangible example of such a failure \mip{mechanism} in modern DRAM is
%\sg{In modern DRAM, this coupling introduces a}
%vulnerability known as 
RowHammer~\cite{kim2014flipping, mutlu2017rowhammer, mutlu2019rowhammer}}.
\sg{RowHammer causes \sg{\emph{disturbance
errors} (i.e., bit flips in \hhs{vulnerable} DRAM cells that are not being accessed)}
in DRAM rows physically adjacent to a row that is repeatedly
activated many times.}}
% Prior works~\cite{tatar2018defeating,
% van2016drammer, gruss2018another, gruss2016rowhammer, razavi2016flip,
% xiao2016one, lipp2018nethammer} develop various system-level
% attacks to \sg{maliciously gain privileged} access by exploiting the RowHammer
% vulnerability.}

\sg{These three challenges are difficult to solve efficiently by directly
modifying the underlying cell array structure.  This is because commodity}
% Optimizing DRAM latency and refresh is a critical challenge as commodity
DRAM implements an extremely dense \emph{DRAM cell array} that is optimized
for \emph{low area-per-bit}~\cite{lee-hpca2013, lee-hpca2015,
son2013reducing}. Because of its density, even a small change in the DRAM
cell array structure may incur \hhs{non-negligible} area
overhead~\cite{lee-hpca2013, udipi2010rethinking, zhang2014half,
mutlu2013memory}. 
\sg{\sgii{\textbf{Our goal} in this work} is to lower the DRAM access latency,
reduce the refresh overhead, and \hhs{improve DRAM reliability} with
\emph{no changes} to the DRAM cell architecture, and with only
\emph{minimal} changes to the DRAM chip.}
% Therefore, it is essential \hho{to lower DRAM latency,
% reduce refresh overhead, and mitigate RowHammer}
% %for a mechanism to require
% \emph{minimal changes} to the DRAM chip, and especially no changes, if
% possible, to the \hh{DRAM cell architecture}. 

% To address \hho{DRAM performance, energy consumption, and reliability} \hhm{challenges}, 
\sg{To this end,} we
propose \hhm{\emph{Copy-Row DRAM (\mech)}}, a flexible in-DRAM substrate that
\sg{can be used in multiple different ways to address the performance, energy
efficiency, and reliability \hhs{challenges} of DRAM.  
The key idea of \mech is to provide a fast, \hha{low-cost} mechanism to
\sgii{\emph{duplicate select rows}} in DRAM that contain data that is most
sensitive \hhs{or vulnerable} to 
latency, refresh, or reliability issues.  \mech}
requires only small changes in commodity DRAM chips.
At a high level, \mech
partitions each DRAM subarray into two regions (\sgii{\emph{regular}} rows and
\sgii{\emph{copy}} rows) and enables independent control over the rows in each region.
The key components required for independent control include 1)~an
independent \hhm{decoder for the \copyrow{s}} and 
%minimal changes 
2)~\hh{small changes in the \sg{memory controller} interface to \hhm{address the
\copyrow{s}}.}
%to the memory controller DRAM interface. 
% Because DRAM rows within the same subarray share \emph{sense amplifiers},
% \hhm{interleaving an access to a \copyrow with an access to a regular row
% results in 
% %unconventional (i.e., non-compliant with the JEDEC
% %specification~\cite{jedec-lpddr4}) but 
% predictable \hho{behavior} between the two rows.
\hho{To store information about the state of the \copyrow{s}
\sg{(e.g., which regular rows are duplicated in which {\copyrow}s)}, \mech
implements a \sg{small} \mech table in the memory controller 
\sg{(Section~\ref{subsec:ctable})}.}


\sg{\mech takes advantage of the fact that DRAM rows in the same subarray
share \emph{sense amplifiers} to enable two \hha{\sgiii{types} of interaction}
between a regular row and a \copyrow.}
First, \sg{\mech can activate (i.e., open)} a \copyrow \emph{slightly
after} \hho{activating} a regular row 
in the same subarray.
Once the \copyrow is activated, the charge restoration
operation in DRAM (used to restore the charge that was drained from the cells of
a row during activation) charges both the regular row \emph{and} the
\copyrow at once.
The simultaneous charge restoration \hhs{of the two rows} \sg{copies the contents of the regular row
into the copy row, similar to the 
in-DRAM row copy operation proposed by
RowClone~\cite{seshadri2013rowclone}.} Second,
\sg{\mech can \emph{simultaneously} activate} a regular \sg{row} and \sg{a} \copyrow 
that \sg{contain} the \hho{\emph{same
data}.} \sg{The simultaneous activation \sgiii{reduces the latency} required to access}
\hho{the data} \sg{by driving each sense amplifier using the charge from \emph{two}
cells \hhs{in each row} (instead of using the charge from only
one cell \hhs{in one row}, as is done in commodity DRAM)}. 

\sg{The \mech substrate is flexible, and can be used to implement
a variety of mechanisms.  In this work}, we
\sg{discuss and evaluate two such novel mechanisms in detail:
1)~\emph{\mech-cache}, which reduces the DRAM access latency
(Section~\ref{subsec:in_dram_caching}) and
2)~\emph{\mech-ref}, which reduces the DRAM refresh overhead
(Section~\ref{subsec:refresh_reduction_mech}).
We \hhs{also} briefly discuss  a third mechanism
that mitigates RowHammer errors (Section~\ref{subsec:crow_hammer}).}
%  \hho{to lower} DRAM access latency
% (Section~\ref{subsec:in_dram_caching})\hho{, reduce}
% refresh overhead (Section~\ref{subsec:refresh_reduction_mech})\hho{, and
% mitigate RowHammer errors (Section~\ref{subsec:crow_hammer})}.}


%unconventional \hh{(i.e., against the JEDEC
%specification~\cite{jedec-lpddr4})} but predictable behavior can be
%observed when interleaving an access to a \copyrow with an access to a
%regular row. 
%Prior work has shown this predictable behavior to be
%exploitable (e.g., RowClone~\cite{seshadri2013rowclone}) \hh{to perform
%in-DRAM bulk copy operations}. Due to its flexibility in interleaving
%accesses to {\copyrow}s and regular rows, the \mech substrate enables
%\hh{RowClone} as well as \hh{two} novel mechanisms that we \hhm{present} in
%\hh{Section~\ref{sec:crow_apps}}. \hh{These are}
%\emph{software-transparent} low-overhead mechanisms that improve DRAM
%performance and energy consumption \hh{by reducing} DRAM access latency and
%refresh overhead.

\sgii{\textbf{Reducing DRAM Access Latency with \mech-cache.}
Prior works\hha{~\cite{hassan2016chargecache, kandemir2015memory, wang2018reducing}} observe
that a significant fraction of the most-recently-accessed rows are
activated again soon after the rows are closed (i.e., the rows exhibit high reuse).
To take advantage of the reuse of recently-accessed rows,
we use \mech to implement \mech-cache, which reduces the DRAM access latency
when a recently-accessed row is activated again.
\textbf{The key idea of \mech-cache} is to
1)~duplicate data from recently-accessed regular rows
into a small cache made up of \copyrow{s}, and
2)~simultaneously activate a duplicated regular row with its corresponding
\copyrow when the regular row needs to be activated again.
By activating both the regular row and its corresponding \copyrow,
\mech-cache reduces the time needed to open the row and begin performing
read and/or write requests to the row by 38\%.}

% \hho{\textbf{\sg{Reducing DRAM Access Latency with \mech-cache}.}}
% \hhm{Prior works~\cite{hassan2016chargecache, kandemir2015memory} observe
% that significant temporal locality} is left unexploited in current DRAM
% architectures (e.g., a significant \hhs{fraction} of recently-closed rows in the
% same bank exhibit high reuse). To take advantage of this unexploited
% locality \sg{to} reduce \sg{the} DRAM access latency, we use \mech to 
% \sg{implement \mech-cache, which provides} a region
% of fast-access memory that we use as an \hhm{\emph{in-DRAM cache}.
% \textbf{\sg{The key idea of \mech-cache}} is to 
% \hhs{1)} \sg{duplicate data from recently-accessed regular rows into a small
% cache made up of {\copyrow}s,
% and \hhs{2)} to simultaneously activate a duplicated regular row with its corresponding
% \copyrow, \hhs{which reduces} the latency required to \hhs{access the data
% duplicated in both rows}.}}
% % use {\copyrow}s to
% % exploit simultaneous activation of multiple rows \hho{(that store the same
% % data)} for reducing activation
% % latency. We efficiently duplicate a frequently-accessed regular row into a
% % \copyrow within the same subarray by activating the \copyrow immediately
% % after the local row buffer latches the data of the regular row. This causes
% % the data from the regular row to be restored to both \hh{the} \copyrow and
% % \hhm{the} regular row.
% % On future accesses \sg{to a cached regular row}, \hhm{\mech-cache} simultaneously
% % activates both \sg{the regular row and its corresponding (which store the same data). 
% \sg{The simultaneous activation enables} \mech-cache to reduce 
% \sg{the activation latency of frequently-accessed rows} by 38\%.
% %  since attaching
% % more DRAM cells with the same charge to a single bitline has an effect
% % similar to driving the bitline with a DRAM cell with a \hhm{larger}
% % capacitance~\cite{choi2015multiple}.

\hho{\textbf{Reducing DRAM Refresh \sg{Overheads with \mech-ref}.}}
\sg{Prior works~\cite{liu2012raidr, liu2013experimental, patel2017reach, qureshi-dsn2015,
hamamoto1998retention, khan-sigmetrics2014} show that only a small
\hha{fraction \hhb{of DRAM cells in a DRAM chip} (e.g., fewer than 1000 cells
in \SI{32}{\gibi\byte} of DRAM~\cite{liu2012raidr})}, \hhb{called \emph{weak}
cells,} \hha{have to} be refreshed at the standard-specified refresh interval
(\SI{32}{\milli\second} in LPDDR4~\cite{jedec-lpddr4}, 
\SI{64}{\milli\second} in DDR3/DDR4~\cite{standard2007ddr3, standard2013ddr4}),
and that \hhs{an overwhelming majority of} cells \hhs{(called \emph{strong}
cells)} can be refreshed much less frequently than the
standard-specified \mip{rate}.
To take advantage of typical-case DRAM cell \hhs{data retention} behavior,
% the longer refresh intervals possible for typical DRAM cells,
we use \mech to implement \mech-ref, which remaps weak \hhs{\emph{regular}} DRAM rows to 
\hhs{strong \emph{copy}} rows.}
% To reduce the performance and energy overhead of the DRAM refresh
% operations, \hhm{we propose \mech-ref, which exploits} the fact that very few DRAM cells actually
% require the JEDEC-specified \hho{\SI{32}{\milli\second}} refresh interval~\cite{jedec-lpddr4,
% liu2012raidr, liu2013experimental, patel2017reach, qureshi-dsn2015,
% hamamoto1998retention}. Our goal is to eliminate the small set of DRAM rows
% with low retention \hhm{times} (\emph{weak DRAM rows}), which can be identified
% via retention time profiling~\cite{patel2017reach, qureshi-dsn2015,
% venkatesan2006retention, khan2016parbor, liu2013experimental,
% khan-sigmetrics2014}.
\sg{\textbf{The key idea of \mech-ref} is to avoid storing any data in DRAM rows
that contain weak cells, such that the \emph{entire} DRAM chip can use a longer refresh
interval.}
% is to extend the refresh \hhm{interval} of a DRAM
% device by \emph{remapping weak DRAM rows to strong {\copyrow}s} \hho{to
% eliminate the few cells that cannot retain their data at extended refresh
% interval}. Due to the tail-end distribution of DRAM cell retention times,
\sg{During system boot or runtime, \mech-ref uses an efficient profiling
mechanism~\cite{patel2017reach} to identify weak DRAM cells, remaps the
\hhs{\emph{regular}} rows containing weak cells to \hhs{strong \emph{copy}} rows, and records the remapping
information in the \mech table.
When the memory controller needs to activate a row, it first
checks the \mech table \hha{to see if the row is remapped, \hhb{and,} if so}, activates the corresponding \copyrow instead of
the regular row.}
% \sg{\mech-ref} \hh{maintains \sg{row remapping} information in
% the \mech-table. 
% Prior to a row activation, the memory controller first
% \hhm{queries} the \mech-table to check whether the row is remapped. If so, the
% memory controller activates the remapped \copyrow instead of the original
% regular row.}
\sg{Because only a very small fraction of DRAM cells are weak,}
remapping only a few \hh{rows} can significantly \sg{reduce the refresh
overhead}, as the weakest DRAM \sg{cell in use} determines the minimum required refresh
rate \sg{of the entire DRAM chip}.
%\sg{Unlike prior works on DRAM refresh reduction~\cite{nair2014refresh,
%qureshi-dsn2015, baek2014refresh, bhati2013coordinated, cui2014dtail,
%emma2008rethinking, ghosh2007smart, isen2009eskimo, jung2015omitting,
%kim2000dynamic, luo2014characterizing, kim2003block, liu2012flikker,
%mukundan2013understanding, nair2013case, patel2005energy,
%stuecheli2010elastic, liu2012raidr}, \mech-ref does \emph{not} require 1)~any
%system software changes to avoid allocating data to DRAM rows with weak
%cells, or 2)~any changes to the conventional DRAM \hhs{}.}
\hhs{\mech-ref has two important properties that prior works~\cite{nair2014refresh,
qureshi-dsn2015, baek2014refresh, bhati2013coordinated, cui2014dtail,
emma2008rethinking, ghosh2007smart, isen2009eskimo, jung2015omitting,
kim2000dynamic, luo2014characterizing, kim2003block, liu2012flikker,
mukundan2013understanding, nair2013case, patel2005energy,
stuecheli2010elastic, liu2012raidr} fail to
\mip{address at the same time}. First, to avoid using weak rows, \mech-ref does \emph{not} require
system software changes that complicate data allocation. Second,
once our \sgii{versatile} \mech substrate is implemented, \mech-ref does not require \sgii{any}
additional changes in DRAM that are specific \sgii{to} enabling a new refresh
scheme.}

% %
%% The remapping scheme (\mech-ref) tracks remapped rows in the \mech-table,
% %which is checked before each row activation. Simply, when a \mech-table
% %entry exists for the row to be accessed, the memory controller activates
% %the remapped \copyrow instead of the original regular row. 
% \hhm{\mech-ref remaps the weak rows based on DRAM retention time
% profiling~\cite{patel2017reach}, which can be performed during system boot
% time or runtime.}
% %
% %The operation of remapping the weak rows \hh{can be} performed \hh{during
% %system boot time} based on \hh{DRAM} retention time
% %profiling~\cite{patel2017reach}. 
% %
% \hho{\sg{\mech allows weak rows to} be remapped dynamically during runtime,} \hhm{which is
% not possible in commodity DRAM chips today}. \mech-ref \hh{significantly}
% reduces the refresh rate and as a result, improves both system performance
% and energy efficiency. \hho{Our approach} \hh{has two key advantages compared to
% prior work on DRAM refresh reduction~\cite{nair2014refresh,
% qureshi-dsn2015, baek2014refresh, bhati2013coordinated, cui2014dtail,
% emma2008rethinking, ghosh2007smart, isen2009eskimo, jung2015omitting,
% kim2000dynamic, luo2014characterizing, kim2003block, liu2012flikker,
% mukundan2013understanding, nair2013case, patel2005energy,
% stuecheli2010elastic, liu2012raidr}.} First, \mech-ref is much simpler to
% implement compared to just disabling access to all the weak rows, because
% \hhm{it does not require changes in the operating system to
% prevent \hho{allocation of} weak rows.}
% %\mech-ref does \emph{not} create holes in the memory address space (see
% %Section~\ref{subsec:refresh_reduction_mech}). 
% Thus, the system can benefit
% from reduced refresh rates without any changes to the software stack.
% Second, \hho{implementing \mech-ref in hardware} \hh{is practical, as it} does \emph{not}
% require any changes to the conventional \hh{DRAM} refresh \hh{circuitry}
% \hhm{(Section~\ref{subsec:remapping_operation})}.


\textbf{Results Overview.} Our evaluations show that 
% \hho{two of} the mechanisms we \hho{propose and} implement, 
\sg{\mech-cache
and \mech-ref} significantly improve performance and energy efficiency. First,
our \sg{access latency reduction mechanism,} \mech-cache, \hhd{provides}
\sg{7.4\% \hhe{higher performance} and consumes 13.3\% less
DRAM energy, averaged across our \hhs{20} memory-intensive four-core workloads,} while reserving
\emph{only} 1.6\% of the DRAM \hha{storage} capacity for {\copyrow}s
\sgii{on a system with four LPDDR4 channels}. Second, our refresh
rate reduction mechanism, \sg{\mech-ref,} \hhe{improves \hhg{system} performance by} \sg{8.1\% and reduces
DRAM energy by 5.4\%, averaged across} the same four-core workloads using the same system
configuration \hha{\sgiii{with} futuristic \SI{64}{\giga\bit} DRAM chips}. \hhm{\mech-cache and \mech-ref} are complementary to
each other. When combined without increasing the number of {\copyrow}s
available, \hhs{the two} mechanisms \hhs{together} improve \sg{average} system performance \hhb{by 20.0\%}
and \hhs{reduce DRAM} energy \hhs{consumption} \hha{by 22.3\%,} \mip{achieving greater improvements 
than either \sgii{mechanism} does alone}.
%\hho{We
%leave the evaluation of the RowHammer mitigation mechanism based on \mech
%as future work.}

\sg{To analyze the activation and restoration
        latency impact of simultaneously activating multiple rows, we
        develop a detailed circuit-level DRAM model.
        %\hhm{that we make
        %publicly available \hhs{along with rest of our simulation
        %infrastructure}~\cite{crow_spice_github}}.
\sgii{We release this circuit-level DRAM model and our simulation infrastructure
that we use to evaluate the performance and energy saving benefits of \mech
as publicly available tools~\cite{crow_spice_github}.}
We hope that this will encourage researchers to develop
other novel mechanisms using the \mech substrate.}

%\mech is a flexible substrate that is not restricted to the two mechanisms that
%we implement and can potentially enable many other mechanisms for improving
%DRAM performance, energy efficiency, and reliability.
%\todo{remove this sentence above?}

\hhs{This paper makes} the following \textbf{key contributions:}
\squishlist

    \item We propose \mech, a flexible and low-cost substrate in
        commodity DRAM that enables mechanisms for improving DRAM
        performance, energy efficiency\hho{, and reliability} by providing two sets of rows
        that have independent control in each subarray. \mech does not
        change the extremely-dense cell array and has \emph{low}
        \hha{cost} (\hhs{0.48\% additional} \hha{area overhead in the DRAM chip,}
        \SI{11.3}{\kibi\byte} \hhs{storage overhead} in the memory
        controller, \hha{and 1.6\% DRAM storage capacity overhead}).
        
    \item We propose \sg{three} mechanisms that \hho{exploit} the \mech
        substrate: 1)~\mech-cache, an in-DRAM cache \sg{to reduce the}
        DRAM access latency\hha{,} 2)~\mech-ref, a remapping scheme for weak
        DRAM rows to reduce the DRAM refresh overhead\hha{,} \hho{and 3)~a
        mechanism for mitigating the RowHammer vulnerability}.
        \hho{We show that \sgii{\mech allows} these mechanisms to be
        employed at the same time.}
 
    \item We evaluate the performance, energy savings, and overhead of
        \hhm{\mech-cache and \mech-ref}, showing significant performance
        and energy benefits \sg{over a \hhs{state-of-the-art} commodity
        DRAM chip}. \hhs{We also compare \mech-cache to \hha{two} prior proposals to
        reduce DRAM latency~\cite{kim-isca2012, lee-hpca2013} and show that
        \mech-cache \sgii{is more area- and energy-efficient at reducing
        \hha{DRAM} latency}.} 

        
\squishend


==> mainmatter/crow/2_background.tex <==
\section{Background}
\label{crow_sec:background}

We describe the low-level organization of DRAM and illustrate how DRAM is
accessed to provide the necessary background for understanding how \mech
operates. We refer the reader to prior work~\cite{kim2012case, zhang2014half,
hassan2016chargecache, lee2013tiered, seshadri2017ambit, chang2017understanding,
chang2016understanding, chang2014improving, chang2016low, lee2015adaptive,
lee2017design, lee2015decoupled, liu2013experimental, liu2012raidr,
seshadri2013rowclone, seshadri2015gather, ipek2008self, lee2016simultaneous} for
a more detailed treatment of various aspects of DRAM operation.

\subsection{DRAM Organization}
\label{crow_sec:bgintro}

A DRAM device is organized hierarchically. The smallest building block, i.e.,
the DRAM cell, consists of a \emph{capacitor} and an \emph{access transistor},
as shown in Figure~\ref{crow_fig:cell}a. The capacitor encodes a single bit of data
by storing different charge levels, i.e., empty or full. During an access to a
cell, the \emph{wordline} enables the access transistor, which connects the cell
capacitor to the \emph{bitline}, so that the cell's state can be read or
modified.


\begin{figure}[t] 
    \centering    
    \includegraphics[width=\linewidth]{figures/crow_dram_cell_sa_bank.pdf}
    \caption{DRAM organization.}
    \label{crow_fig:cell}
\end{figure}


A \emph{subarray} consists of a 2D array of DRAM cells, as shown in
Figure~\ref{crow_fig:cell}b. The cells that share the same wordline in a subarray
are referred to as a DRAM \emph{row}.  Each subarray is typically composed of
512--1024 rows. To prepare a row for an access, the \emph{local row decoder}
selects the row by enabling the corresponding wordline in the subarray. In
conventional DRAM, only one row in a subarray can be enabled at a time, and,
thus, only one cell is enabled on each bitline. When a cell is enabled,
\emph{charge sharing} takes place between the cell and the bitline (which is
initially \emph{precharged} to a reference voltage). This charge sharing shifts
the bitline voltage up or down based on the voltage of the cell. The bitline's
\emph{sense amplifier} detects the bitline voltage shift and amplifies it to a
full 0 or 1 (i.e., $V_{ss}$ or $V_{dd}$). All sense amplifiers that detect and
amplify the charge levels of the cells of the open row inside a subarray are
referred to as the subarray's \emph{local row buffer}. 

As illustrated in Figure~\ref{crow_fig:cell}c, multiple subarrays are organized into
a group to form a \emph{bank}. To select a particular row, the memory controller
sends the row address to the \emph{global row decoder}, which partially decodes
the address to select the local row decoder of the subarray that contains the
row. Each bank includes a \emph{global row buffer}. On a read operation, the
requested portion of the target row is copied from the local row buffer of the
subarray that contains the target row into the global row buffer. Once this is
done, the global row buffer sends its data to the memory controller.

A single DRAM \emph{chip} contains multiple banks that operate in parallel. To
provide high bandwidth, multiple chips are grouped together into a \emph{rank}.
The chips in a rank share the same address/command bus, which causes the chips
to operate in lockstep (i.e., the chips receive the same commands and perform
the same operations on different portions), but each chip has its own data bus
connection. To increase the system's total memory capacity, multiple ranks are
connected to the same DRAM \emph{channel}, operating in a time-multiplexed
manner by sharing the channel bus (i.e., address/command/data pins). In a
typical system, each memory controller interfaces with a single DRAM channel and
sends addresses/data/commands over the channel bus to manipulate the data stored
within all ranks that are part of the channel. 

\subsection{DRAM Operation}
\label{crow_subsec:dram_op}

There are four major commands that are used to access DRAM: \cmdact, \cmdwrite,
\cmdread, and \cmdprech. DRAM command scheduling is tightly regulated by a set
of \emph{timing parameters}, which guarantee that enough time has passed after a
certain command such that DRAM provides or retains data correctly.
Figure~\ref{crow_fig:latency} illustrates the relationship between the commands
issued to perform a DRAM read and their governing timing parameters. The memory
controller enforces these timing parameters as it schedules each DRAM command.
Aside from the DRAM access commands, the memory controller also periodically
issues a \cmdrefresh command to prevent data loss due to leakage of charge from
the cell capacitors over time.


\begin{figure}[h] 
    \centering
    \includegraphics[width=0.9\linewidth]{figures/DRAM_latency_operation.pdf} 
    \caption{Commands, timing parameters, and cell/bitline voltages during a DRAM read operation.}
    \label{crow_fig:latency}
\end{figure}

\textbf{Activate (\cmdact).} 
The \cmdact command \emph{activates} (opens) a DRAM row by transferring the data
contained in the cell capacitors to the row buffer. \cmdact{} latency is
governed by the \trcd{} timing parameter, which ensures that enough time has
passed since the \cmdact is issued for the data to stabilize in the row buffer
(such that it can be read). 

\cmdact consists of two major steps: 1) capacitor-bitline \emph{charge sharing}
and 2) \emph{charge restoration}. Charge sharing begins by enabling the wordline
(\circled{1} in Figure~\ref{crow_fig:latency}), which allows the cell capacitor to
share charge with the bitline, and thus perturb the precharged bitline voltage.
Once the cell and bitline voltages equalize due to charge sharing, charge
restoration starts (\circled{2}). During charge restoration, the sense
amplifiers are enabled to first detect the bitline voltage shift, and later
restore the bitline to a full $V_{ss}$ or $V_{dd}$ depending on the direction of
the shift. Once the bitline is restored to a \emph{ready-to-access} voltage
level (\circled{3}), restoration is complete, and the other DRAM commands (e.g.,
\cmdread, \cmdwrite) can be issued to the bank.


\textbf{Read (\cmdread).}
After a row activation, the memory controller reads data from the open row by
issuing an \cmdread command. The \cmdread includes a column address, which
indicates the portion of the open row to be read. When a DRAM chip receives an
\cmdread command, it first loads the requested portion of the open row into the
global row buffer. After the data is in the global row buffer, the DRAM chip
sends the data across the data bus to the memory controller. The \cmdread{}
command is governed by the timing parameter \tcl, after which the data appears
on the data bus.


\textbf{Write (\cmdwrite).}
The \cmdwrite command (not shown in Figure~\ref{crow_fig:latency}) modifies data in
an open DRAM row. The operation of \cmdwrite is analogous to \cmdact in that
both commands require waiting enough time for the sense amplifiers to restore
the data in the DRAM cells.  Similar to how a sense amplifier restores a cell
capacitor during the second step of \cmdact, in case of a \cmdwrite, the sense
amplifier restores the capacitor with the new data value that the \cmdwrite
command provides. The restoration latency for \cmdwrite is governed by the \twr
timing parameter. For both \cmdact and \cmdwrite commands, the restoration
latency originates from the sense amplifier driving a bitline to replenish the
charge of the DRAM cell
capacitor~\cite{kim2012case,kang2014co,lee2015adaptive,zhang2015exploiting}.
This makes any optimizations to the charge restoration step of \cmdact equally
applicable to \cmdwrite. Thus, using such optimizations we can decrease both
\tras and \twr.

\textbf{Precharge (\cmdprech).} 
\cmdprech is used to \emph{close} an open DRAM row and prepare the DRAM bank for
activation of another row. The memory controller can follow an \cmdact with
\cmdprech to the same bank after at least the time interval specified by \tras.
\tras ensures that enough time has passed to fully restore the DRAM cells of the
activated row to a \emph{ready-to-precharge voltage} (\circled{4} in
Figure~\ref{crow_fig:latency}). The latency of \cmdprech is governed by the timing
parameter \trp, which allows enough time to set the bitline voltage back to
reference level (e.g., $V_{dd}/2$). After \trp, the memory controller can issue
an \cmdact to open a new row in the same bank.

\textbf{Refresh (\cmdrefresh).} 
A DRAM cell cannot store its data permanently, as the cell capacitor leaks
charge over time. The \emph{retention time} of a DRAM cell is defined as the
length of time for which the data can still be correctly read out of the cell
after data is stored in the cell. To ensure data integrity, the memory
controller periodically issues \cmdrefresh commands to the DRAM chip. Each
\cmdrefresh command replenishes the charge of several DRAM rows starting from
the one that a \emph{refresh counter} (implemented in the DRAM chip) points to.
The memory controller is responsible for issuing a sufficient number of
\cmdrefresh commands to refresh the entire DRAM during a manufacturer-specified
refresh interval (typically \SI{64}{\milli\second} in DDR3 and DDR4 DRAM, and
\SI{32}{\milli\second} in LPDDR4).


==> mainmatter/smd/sections/0_abstract.tex <==
\begin{abstract}
    % \vspace{-10pt}

    The rigid interface of current DRAM chips \hht{places the memory controller
    completely in charge of DRAM control}. Even DRAM maintenance operations,
    which are used to ensure correct operation (e.g., refresh) and combat
    reliability/security issues of DRAM (e.g., RowHammer), are managed by the
    memory controller. \hht{Thus}, implementing new \agy{maintenance operations}
    or modifying the existing \agy{ones} often require \hh{difficult-to-realize}
    \agy{\hht{changes} in the} DRAM interface, memory controller\agy{,} and
    potentially other system components \hht{(e.g., system software), leading to
    slow progress in DRAM systems}.
    %
    % \hh{For example, the cost of offering a new refresh mode, improved RowHammer
    % protection, and in-DRAM memory scrubbing as part of the new DDR5 standard
    % spanned 1) multiple years for development of the standard and 2) adopting
    % the standard in DRAM chip and memory controller designs. To enable fast
    % adoption of new and efficient DRAM maintenance operations, there is a need
    % for constraining the changes required to implement the maintenance operation
    % to a DRAM chip.}

    % All these new features are enabled with new
    % DRAM commands that require changes in the DRAM interface and the memory
    % controller.

    % We argue that enabling support for autonomous maintenance mechanisms in
    % DRAM would make adopting new ideas for efficient maintenance operations
    % easier and enable quickly deploying mitigation mechanisms for newly
    % discovered DRAM vulnerabilities. 
    In this paper, our goal is to \hh{1) \bgyellow{ease, and thus accelerate,}
    the process of \hhf{enabling} new DRAM maintenance operations and 2) enable
    \hht{more} efficient in-DRAM maintenance operations. \hht{Our idea is to
    set} the memory controller free from managing DRAM maintenance}. To \hh{this
    end}, we propose \mechlong{} (\mech{}), a new low-cost DRAM architecture
    that enables implementing new in-DRAM maintenance mechanisms \hht{(or
    modifying old ones)} with no further changes in the DRAM interface, memory
    controller, or other system components. 
    % The key idea of \mech{} is to allow a DRAM chip to internally perform a
    % maintenance operation on a DRAM region while preventing the memory
    % controller from accessing this region until the maintenance operation
    % completes. 
    \hh{We use \mech{} to implement \hhf{new in-DRAM} maintenance mechanisms for
    three use cases: 1) periodic refresh, 2) RowHammer protection, and 3) memory
    scrubbing}. 
    %
    % Our evaluations show that, when used in combination, our maintenance
    % mechanisms provide 7.6\% performance improvement compared to \agy{a
    % baseline} with no RowHammer protection and memory scrubbing. 
    %
    \bgyellow{We show that \mech{} enables easy adoption of efficient maintenance
    mechanisms that} significantly \hht{improve the} system performance and
    energy \hht{efficiency} \hhf{while providing higher reliability} compared to
    conventional DDR4 DRAM. 
    % \hht{For example, 1)} \mech{}-based periodic refresh
    % achieves 19.5\% speedup and 11.5\% lower DRAM energy consumption on average
    % for four-core workloads. \hht{2) \mech{}-based RowHammer protection and
    % memory scrubbing improve DRAM reliability and security with low performance
    % and energy overheads compared to mechanisms implemented in existing DRAM
    % chips.}
    %
    % We believe that providing a DRAM
    % chip the ability to internally and autonomously perform maintenance
    % operations would encourage the innovation and reduce time-to-market for new
    % mechanisms that improve DRAM \hh{efficiency,} reliability, and security. 
    %
    % We believe this approach
    % reduces the time-to-market for new DRAM mechanisms for improving DRAM
    % refresh and mitigating new DRAM vulnerabilities.
    %
    \hhf{A combination of \mech{}-based maintenance mechanisms that perform
    refresh, RowHammer protection, and memory scrubbing achieve 7.6\% speedup
    and 5.2\% lower DRAM energy on average for four-core workloads.}
    

\end{abstract}


==> mainmatter/smd/sections/1_intro.tex <==
% !TEX root=../main.tex

%\vspace{-2mm}

\section{Introduction}
\label{sec:intro}
% \vspace{-10pt}

% why is DRAM important and
% reliability problems of DRAM: retention, VRT, particle strikes, rowhammer
DRAM is \agy{the prevalent \hh{main} memory technology used} in \hh{almost all}
computer systems. Advances in manufacturing technology and DRAM design enable
increasingly smaller DRAM cell \hht{sizes}, continuously reducing cost per bit
of a DRAM chip~\cite{lee2017design,mutlu2013memory, mutlu2014research,
nair2013archshield}. However, as a DRAM cell becomes smaller and the distance
between adjacent cells shrink, ensuring reliable \hh{and efficient} DRAM
operation \hht{becomes} an even more critical
challenge\cite{awasthi2012efficient,cha2017defect,hong2010memory,kang2014co,kim2020revisiting,kim2014flipping,
lee2016technology, mandelman2002challenges, mutlu2013memory,
mutlu2019rowhammer,nair2013archshield, park2015technology,qureshi2015avatar}. A
modern DRAM chip typically requires three types of maintenance operations for
reliable and secure operation: 1) DRAM refresh, 2) RowHammer protection, and
3) memory scrubbing.\footnote{Memory scrubbing is not \hht{always} required in
consumer systems but often used by cloud service
providers~\cite{jacob2010memory,
mukherjee2004cache,schroeder2009dram,meza2015revisiting, saleh1990reliability,
siddiqua2017lifetime, micron2019whitepaper, gong2018duo}.}

% A DRAM
% cell consists of a single \emph{access transistor} and \emph{storage capacitor}.
% Although such a design provides high bit density and low access latency, it
% suffers from the retention problem due to charge leakage in DRAM cells.

% the retention problem of DRAM and refresh
\textbf{DRAM Refresh.} Due to the short retention time of DRAM cells, \hh{all
DRAM cells need to be periodically refreshed} to ensure reliable operation. In
existing DRAM chips, a cell is typically refreshed every 64 or
\SI{32}{\milli\second} \hh{below
\SI{85}{\celsius}~\cite{micronddr4,ddr4,2014lpddr4} and every
\SI{16}{\milli\second} above \SI{85}{\celsius}~\cite{lpddr5,jedec2021ddr5}}. \hht{A} DRAM
chip consists of billions of cells, and therefore refreshing such a large number
\agy{of} cells incurs \hht{large} performance and energy
overheads~\cite{liu2012raidr, liu2013experimental, qureshi2015avatar}. These
overheads \agy{are} expected to increase as DRAM chips become
denser~\cite{chang2014improving,kang2014co,liu2012raidr}. \hht{Many ideas have
been proposed} to mitigate \hht{the} DRAM refresh
overhead~\cite{chang2014improving, liu2012raidr,
qureshi2015avatar,nair2014refresh, baek2014refresh, bhati2013coordinated,
cui2014dtail, emma2008rethinking, ghosh2007smart, isen2009eskimo,
jung2015omitting, kim2000dynamic, luo2014characterizing, kim2003block,
liu2012flikker, mukundan2013understanding, nair2013case, patel2005energy,
stuecheli2010elastic, khan2014efficacy, khan2016parbor, khan2017detecting,
venkatesan2006retention, patel2017reaper, riho2014partial, hassan2019crow,
kim2020charge, nguyen2018nonblocking, kwon2021reducing}.


% To ensure data integrity, DRAM standards (e.g., DDR4, LPDDR4, GDDR6) specify a
% refresh period (typically \SI{64}{\milli\second}), which indicates the time
% interval during which the charge of each DRAM cell capacitor must be replenished
% at least once. In addition to consuming energy, DRAM refresh operations also
% negatively impact system performance as a DRAM bank cannot be accessed while
% being refreshed. As technology nodes shrink and DRAM cells become smaller, DRAM
% retention comes out as an increasingly more challenging problem to solve during
% DRAM design and manufacturing, even requiring more frequent periodic
% refresh~\cite{}. 


% the RowHammer problem of DRAM and RowHammer Protection Mechanisms
\textbf{RowHammer Protection.} 
%
% First reported in 2014 by Kim et
% al.~\cite{kim2014flipping}, small and densely packed DRAM cells suffer from
% \emph{RowHammer}, which causes DRAM disturbance failures that stem from the
% electro-magnetic interference caused by repeatedly activating (i.e., hammering)
% a DRAM row \agy{(i.e., aggressor row)} many
% times~\cite{redeker2002investigation,yang2019trap,gautam2019row,jiang2021quantifying,park2016experiments,
% park2016statistical, ryu2017overcoming, walker2021dram,yang2016suppression}.
%
% \hh{In 2014, Kim et al.~\cite{kim2014flipping} reported that small and densely
% packed DRAM cells suffer from the \emph{RowHammer} vulnerability.} 
\hh{\hht{Small and densely-packed DRAM cells suffer from the RowHammer
vulnerability~\cite{kim2014flipping}, which leads to} disturbance failures that
stem from electro-magnetic interference created by repeatedly activating (i.e.,
hammering) a DRAM row (i.e., aggressor row) many
times~\cite{yang2019trap,gautam2019row,jiang2021quantifying,park2016experiments,
park2016statistical, ryu2017overcoming, walker2021dram,yang2016suppression}.}
\hh{Such rapid row activations lead to bit flips in DRAM rows that are
physically nearby an aggressor row}. Many works propose mechanisms to protect
DRAM chips against RowHammer~\cite{rh-apple,kim2014flipping,
aweke2016anvil,kim2021mithril,lee2019twice,park2020graphene,seyedzadeh2017counter,son2017making,taouil2021lightroad,yauglikcci2021security,you2019mrloc,
yaglikci2021blockhammer,greenfield2016throttling,
hassan2019crow,saileshwar2022randomized, konoth2018zebram,
brasser2016can,van2018guardion, marazzi2022protrr, kim2022mithril}.

%Today, a widely-used approach to mitigate RowHammer failures
% is to refresh the adjacent rows upon detecting a row that is being hammered.
% These approaches further increase the performance and energy overhead of the
% DRAM refresh operations.

% random DRAM bit errors in DRAM: VRT and particle strikes AND ECC
\textbf{Memory Scrubbing.}
\hh{System designers typically use Error Correcting Codes
(ECC)~\cite{hamming1950error,dell1997white} to improve \hht{system} reliability.
\bgyellow{Moreover, DRAM vendors equip DRAM chips with on-die ECC to improve
factory yield}~\cite{jedec2021ddr5, patel2019understanding, patel2020bit,
patel2021harp, nair2016xed}. 
% An ECC scheme uses redundancy to encode a data chunk into a
% codeword. Bit errors that occur in a codeword stored in DRAM can be detected and
% corrected upon decoding the codeword. 
\hht{Detection} and correction capability of an ECC scheme is limited. For
example, \emph{Single-Error-Correction Double-Error-Detection (SECDED)} ECC
detects up to two bit errors and corrects one bit error in a codeword. To
prevent \hht{independent} single-bit errors from accumulating \hhf{into}
multi-bit errors, memory scrubbing~\cite{jacob2010memory,
mukherjee2004cache,schroeder2009dram,meza2015revisiting, saleh1990reliability,
siddiqua2017lifetime, micron2019whitepaper, gong2018duo} is \hht{commonly employed:
the entire memory is scanned to correct single-bit errors.}}
%  by decoding and encoding codewords in DRAM.}


% A vast majority of cells in a DRAM chip normally retain their data for much
% longer than the designated refresh period\cite{khan2014efficacy,
% liu2013experimental,patel2017reaper}. However, due to a phenomenon known as
% Variable Retention Time (VRT)~\cite{qureshi2015avatar,
% liu2013experimental,restle1992dram,yaney1987meta}, some DRAM cells can switch
% between low and high retention modes at arbitrary time. Consequently, a DRAM
% cell that remains in high retention mode during testing may switch to low
% retention mode and introduce a bit error at runtime. Various other factors
% (e.g., particle strikes, electromagnetic interference) can cause a bit flip in
% DRAM~\cite{kang2014co,
% kwon2014understanding,liu2013experimental,meza2015revisiting,nair2016xed,son2015cidra}.
% System designers typically use Error Correcting Codes
% (ECC)~\cite{hamming1950error,dell1997white} to protect DRAM against such errors.
% Recently, DRAM vendors even started \agy{to} equip their DRAM chips with on-die
% ECC~\cite{ddr5, patel2019understanding, patel2020bit, patel2021harp,
% nair2016xed}. Besides applying error correction when reading data from DRAM, ECC
% is also widely used to perform periodic memory scrubbing~\cite{jacob2010memory,
% mukherjee2004cache,schroeder2009dram,meza2015revisiting, saleh1990reliability,
% siddiqua2017lifetime, micron2019whitepaper, gong2018duo} to prevent the accumulation
% of single-bit errors that may turn into uncorrectable (and even undetectable)
% multi-bit errors.

% a paragraph that argues DRAM requires a good amount of maintenance
% The maintenance operations incur significant performance and energy overhead
% besides, due to the rigid interface of DRAM, it is difficult to modify
% existing maintenance operation or introduce new ones.

We consider periodic refresh, RowHammer protection, and memory scrubbing as
\emph{DRAM maintenance operations} needed for reliable and secure operation of
modern \hht{and future} DRAM \agy{chips}. \hh{An ideal maintenance operation
should efficiently improve DRAM reliability and security \hht{with} minimal
system performance and energy consumption \hht{overheads}.}

\hh{\hht{As} DRAM technology node \hht{scales to smaller sizes}, the reliability
and security of DRAM chips worsen. As a result, new DRAM chip \hht{generations
necessitate} making existing maintenance operations more \bgyellow{aggressive}
(e.g., lowering the refresh period~\cite{jedec2021ddr5, lpddr5, rh-apple}) and
introducing new types of maintenance operations (e.g., targeted
refresh~\cite{hassan2021uncovering,frigo2020trrespass,jattke2022blacksmith}
\hht{and DDR5 RFM~\cite{jedec2021ddr5} as RowHammer defenses}). As the intensity
and number of different maintenance operations increase, it becomes increasingly
more challenging to keep the overhead of the maintenance operations low.}

\hh{Unfortunately, modifying the DRAM maintenance operations is difficult due}
to the current rigid DRAM interface that \hht{places the Memory Controller (MC)
completely in charge of DRAM control}. \bgyellow{Implementing new maintenance
operations (or changing existing ones) often necessitate modifications in the
DRAM interface, MC, and potentially other system components. Such modifications
are only possible with a new DRAM standard, which takes a long time to develop,
leading to slow progress in DRAM systems. For example, there was a five-year gap
between the DDR3~\cite{jedec2008ddr3} and DDR4~\cite{ddr4} standards, and
eight-year gap between the DDR4~\cite{ddr4} and DDR5~\cite{jedec2021ddr5}
standards. In addition to waiting for a new standard to come out, DRAM vendors
also need to push their proposal regarding the maintenance operations through
the JEDEC committee so the new standard includes the desired changes to enable
new maintenance operations. Thus, we believe a flexible DRAM interface that
allows DRAM vendors to quickly implement custom in-DRAM maintenance mechanisms
would help to develop more reliable and secure DRAM chips.}

% Implementing new or modifying existing
% maintenance operations often require \hht{difficult-to-realize} \agy{changes in}
% the DRAM interface\agy{,} the MC\agy{,} and other system components \agy{(e.g.,
% \hht{system software})}. For example, the new DDR5 standard~\cite{jedec2021ddr5}
% introduces three major changes to optimize and improve DRAM maintenance
% operations. \hh{These changes are difficult to implement \hht{as} they were only
% possible by developing the new DDR5 standard with multi-year
% effort\footnote{DDR5 specification~\cite{jedec2021ddr5} was released in 2021, 9 years
% after the release of the DDR4 specification~\cite{ddr4}.} from \hht{many}
% parties that are part of the JEDEC committee.}


% \textbf{Our goal} is to enable \emph{flexibility} in designing DRAM maintenance
% operations such that DRAM vendors can quickly deploy their new solutions or
% modifications without necessarily demanding changes in the DRAM standards,
% MCs, or other system components. 

\textbf{Our goal} is to \hht{1) ease\bgyellow{, and thus accelerate,} the
process of implementing new DRAM maintenance operations and 2) enable more
efficient in-DRAM maintenance operations.} \hh{We believe that enabling
\hht{autonomous} in-DRAM maintenance operations would encourage innovation\hht{,
reduce} time-to-market, \hht{and ease adoption of novel} mechanisms that improve
DRAM efficiency, reliability, and security. DRAM architects will quickly deploy
their new in-DRAM solutions to tackle reliability and security problems of DRAM
without demanding further changes in the DRAM interface, MC, or other system
components.}
%
% explain how we achieve the goal



We propose \mechlong{} (\mech{}), a new DRAM architecture that enables DRAM
vendors to implement new maintenance operations and modify the existing ones
without the need to make further changes in the DRAM interface, MC, or other
system components. 
% The \textbf{key idea} of \mech{} is to make a DRAM chip manage itself by
% moving the control of maintenance operations from the MC to the
% DRAM chips. 
\bgyellow{Using \mech{}, DRAM vendors can rapidly implement new solutions to cope
with the increasing reliability and security problems of DRAM without the need
of a new DRAM standard.}

The \textbf{key idea} of \mech{} is to allow a DRAM chip to \hht{autonomously}
perform maintenance operations \hht{by preventing memory} accesses to DRAM
regions \hht{that are} under maintenance. To prevent access to a DRAM region
under maintenance \hht{(e.g., specific DRAM banks)}, \hh{an \mech{} chip
\agy{\emph{rejects}}} a row activation command (i.e., \cmdact{}) issued by the
MC. \hh{After the DRAM chip completes the maintenance operation, \hht{the MC
re-issues an} \cmdact{} to the same row}.


% the requirements that a maintenance mechanism should satisfy
\hh{An \mech{}} chip autonomously performs maintenance operations. For example,
the MC \hht{never issues} \cmdrefresh{} commands to \hht{an \mech{}} chip.
\hht{In fact, the MC does \emph{not} even know which maintenance operations an
\mech{} chip performs.} In general, a maintenance mechanism in an \mech{} chip
operates in three steps. First, the maintenance mechanism \emph{locks} a
\agy{DRAM} region \hht{where it will} perform maintenance. \mech{} prevents the
MC from accessing the locked region \hh{by rejecting row activation
\hht{commands} (i.e., \cmdact{}) that \hht{target}} the locked region.
%the locked region by rejecting row activations. 
Second, the maintenance mechanism performs a maintenance operation,
\bgyellow{i.e.,} refreshes rows within the region, \hht{performs RowHammer
mitigation}\bgyellow{, or corrects bit flips via scrubbing}. Third, \hh{after
completing the maintenance, the maintenance mechanism releases the locked DRAM
region to allow the MC to access it}.


% the high level changes in the DRAM interface to enable SMD
\hh{To enable practical adoption of \mech{}, we implement it with low-cost
modifications in existing DRAM chips and MCs.} \mech{} requires simple changes
in the MC to enable re-issuing a previously-rejected \cmdact{} command,
\bgyellow{but at the same time it} simplifies MC design as \bgyellow{the MC} is
no longer responsible for managing DRAM maintenance operations.
%
\hht{First, to inform the MC that a row activation is rejected,
\mech{} adds a single uni-directional pin to a DRAM chip. Second, in a DRAM
chip, \mech{} implements a \emph{Lock Controller} for managing regions under
maintenance and preventing access to them. In \cref{sec:hw_overhead}, we
show that the core components of \mech{} have low DRAM chip area overhead
(1.63\% of a \SI{45.5}{\milli\meter\squared} DRAM chip) and latency cost
(\emph{only} 0.4\% additional row activation latency).}
% \footnote{\hht{A
% maintenance mechanism may require additional area to implement its components.
% Note that the same area will be needed also when implementing the maintenance
% mechanism without \mech{} by changing the DRAM interface.}} 
% Third, although \mech{} requires simple changes in the MC to enable re-issuing a
% previously-rejected \cmdact{} command, \mech{} simplifies MC design as it is no
% longer responsible for managing DRAM maintenance operations.}

% In general, a maintenance mechanism must satisfy two requirements to
% ensure correct DRAM operation. First, a maintenance mechanism should lock (using
% the subarray locking mechanism that \mech{} provides) the subarray or subarrays
% to prevent the MC from accessing these subarray during the
% maintenance operation. The maximum number of subarrays that a maintenance
% mechanism can lock in a bank depend on the design of \mech{} as we discuss in
% Section~{\todo{add crossref}}. Second, a maintenance operation should not lock
% other subarrays for the \emph{Timeout Duration (TD)} after communicating the
% addresses of the currently locked subarrays to the MC. This
% requirement is needed to correctly synchronize the MC and the
% DRAM chip on which subarrays are locked. Since the communicated locked subarray
% information remains valid in the MC for \emph{TD}, only after
% \emph{TD} the DRAM chip can lock new subarrays as the MC is not
% able to access the bank without querying the new locked subarrays.


% explain the maintenance mechanisms we implement in this paper
We demonstrate the versatility \hht{and example benefits} of \mech{} by
implementing maintenance mechanisms for three use cases: \agy{1)~}periodic
refresh, \agy{2)~}RowHammer protection, and \agy{3)~}memory scrubbing. 

First, we implement two maintenance mechanisms for DRAM refresh.
\emph{Fixed-Rate Refresh} \hht{(\fr{})} uniformly refreshes the entire DRAM chip
at a fixed refresh period. Compared to conventional DRAM refresh, our approach
\hht{has the benefit of allowing} \hht{accesses to DRAM regions that are not
being refreshed}. \emph{Variable Refresh} \hht{(\vr{})} refreshes DRAM rows with
different periods based on \hht{the data} retention capability of each row\hht{,
further lowering the refresh overheads}. 

Second, we implement \hext{three} maintenance mechanisms for RowHammer
protection. \emph{Probabilistic RowHammer Protection} \hht{(\prp{})} protects a
DRAM chip against RowHammer by refreshing the neighbors of an activated row with
a low probability. \hht{\prpplus{}} uses area-efficient Bloom Filters to
identify potential aggressor rows and refresh the neighbors of only \hht{such
rows, eliminating unnecessary neighbor row refreshes when the activation count
of an aggressor row is low}. \hext{\drp{} is a deterministic RowHammer
protection mechanism that keeps track of the most-frequently activated DRAM rows
and refreshes their neighbors when activated more than a certain threshold.}
\hht{Existing DRAM chips use on-die Target Row Refresh (TRR) that piggybacks
TRR-induced refreshes to regular refresh commands, which does not incur
performance overhead but provides limited time for RowHammer
protection~\cite{hassan2021uncovering,jattke2022blacksmith,frigo2020trrespass}.
Compared to TRR, \prp{}, \prpplus{}, \hext{and \drp{}} can be configured to
efficiently refresh neighbor rows at the desired rate to strengthen the
RowHammer protection.} 

Third, we implement \emph{Memory Scrubbing} \hht{(\sms{})}, \hht{which scans the
DRAM at a fixed time interval} to correct single-bit errors. Compared to
conventional memory scrubbing that is performed by the MC, \sms{}
has significantly lower scrubbing overhead, especially at low scrub periods
(e.g., $\leq 1~minute$).

\hht{We demonstrate the implementation of six example \mech{} maintenance
mechanisms that resemble mechanisms implemented in existing DRAM chips. However,
\mech{} chip designers have the freedom to implement different maintenance
mechanisms without exposing any information to the MC or other
system components.}

% summarize the results
Our evaluations show \hh{the efficiency of \mech{}-based DRAM maintenance
mechanisms}. \hh{When using \SI{32}{\milli\second} \hht{(\SI{16}{\milli\second})}
refresh period,} \fr{}/\vr{} provides \hh{8.7\%/9.2\%} \hht{(19.5\%/20.7\%)}
\hh{average speedup} compared to conventional DDR4 refresh for memory-intensive
four-core workloads, achieving \hh{86.8\%/91.2\%} \hht{(86.6\%/92.3\%)} of
performance provided by a hypothetical DRAM that does not require any refresh.
When combined, \vr{}, \prp{}, and \sms{} \hh{still} provide \hh{7.6\%}
\hht{(19.0\%)} \hh{speedup compared to} the DDR4 baseline, showing that the
performance overhead of \hh{\mech{}-based} RowHammer protection and memory
scrubbing is small.
% such that it still outperforms the DDR4 baseline with no RowHammer protection and
% memory scrubbing. 
Due to reduced execution time and low \hh{maintenance operation} overhead,
\vr{}, \prp{}, and \sms{} consume \hh{5.2\%} \hht{(12.0\%)} less DRAM energy
compared to the DDR4 baseline.

% We demonstrate the versatility of \mech{} by implementing \agy{five new DRAM}
% maintenance mechanisms for three use case\agy{s}. 
%In addition to these, we discuss other use cases in Section~\ref{subsec:other_use_cases}. 
We \agy{expect and} hope that \mech{} will inspire researchers to develop new
DRAM maintenance mechanisms and enable practical adoption of innovative ideas by
\hht{providing freedom to both DRAM and MC designers}. We will
publicly release all \mech{} source code and data.


We make the following \textbf{key contributions}:
\squishlist
    \item We propose \mech{}, \hh{a new DRAM chip design \hht{and interface} to
    enable autonomous and efficient in-DRAM} maintenance operations. We
    implement \mech{} with small changes \hht{to modern} DRAM chips and MCs.
    %  while largely preserving the existing DRAM standards (e.g.,
    % DDRx, LPDDRx).

    \item We use \mech{} to implement \hh{efficient} DRAM maintenance mechanisms
    for three use cases: DRAM refresh, RowHammer protection, and memory
    scrubbing. 
    % We discuss DRAM error profiling and
    % processing-in-memory as other use cases for \mech{}.

    \item We rigorously evaluate the performance and energy of the new
    maintenance mechanisms. \hht{\mech{} provides large performance and energy
    benefits while also improving reliability across a variety of systems and
    workloads.}

\squishend 

==> mainmatter/smd/sections/2_background.tex <==
\section{Background}
\label{sec:background}
% \vspace{-10pt}

\hht{We provide a brief background on DRAM.}

% explain DRAM Organization with a focus on subarrays and local decoders/rowbuffers
\subsection{DRAM Organization}
\label{subsec:dram_organization}
% \vspace{-10pt}

A typical computing system has one or more \emph{DRAM channels}, where each
channel has an independently operating I/O bus. As
Fig.~\ref{fig:dram_organization} illustrates, a \hht{Memory Controller (MC)}
interfaces with one or multiple \emph{DRAM ranks} via the channel's I/O bus. A
DRAM rank consists of a group of DRAM chips that operate in lockstep. Because
the I/O bus is shared across ranks, accesses to different ranks happen in serial
manner. A DRAM chip is divided into multiple \emph{DRAM banks}, each of which is
further divided into multiple two dimensional DRAM cell arrays, called
\emph{subarrays}. Within each subarray, DRAM cells are organized as \emph{rows}
and \emph{columns}. A DRAM cell connects to a \emph{sense amplifier} via a
\emph{bitline}, and all sense amplifiers in the subarray form a \emph{row
buffer}. Within each DRAM cell, the data is stored as \emph{electrical charge}
on the capacitor and accessed through an \emph{access transistor}. To perform a
DRAM access, a row first must be activated (i.e., opened), which loads row's
data into the row buffer. A row activation is performed by enabling the
\emph{wordline} that corresponds to the row address that the MC provides along
with the \cmdact{} command. To enable the corresponding wordline, the
\emph{global row decoder} first partially decodes the row address, and the
\emph{local row decoder} selects a wordline based on the partially decoded
address provided by the global row decoder.

% the source file of the figure: https://www.figma.com/file/38SnEuvjWtkvgwADRTs4QZ
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{figures/dram_organization.pdf}
    \caption{A typical DRAM-based system.}
    \label{fig:dram_organization}
\end{figure}

% briefly explain the commands for accessing DRAM
\subsection{Accessing DRAM}
\label{subsec:accessing_dram}
% \vspace{-10pt}

\bgyellow{To perform a DRAM access, a row first must be activated (i.e.,
opened), which loads row's data into the row buffer. A row activation is
performed by enabling the wordline that corresponds to the row address that the
\cmdact{} command. To enable the corresponding wordline, the \emph{global row
decoder} first partially decodes the row address, and the \emph{local row
decoder} selects a wordline based on the partially decoded address provided by
the global row decoder.}

\bgyellow{Once a wordline is enabled, the row activation process (i.e., loading
rows' data into the row buffer) occurs in two steps. First, each cell in the
activating row share its charge with the corresponding bitline.} Due to the
charge sharing, the bitline voltage slightly deviates from its pre-activation
voltage level. Second, a sense amplifier detects the bitline voltage deviation
and gradually restores the cell capacitor back to its original charge level. The
data in the row buffer becomes accessible by a \cmdread{}/\cmdwrite{} command
when the bitline and cell voltage is restored to a certain level. Therefore, the
MC should follow an \cmdact{} with one or multiple \cmdread{}/\cmdwrite{}
\hht{commands} at least after the \emph{activation latency} (\trcd{}). 

\bgyellow{The MC issues a \cmdpre{} command to close an open row, after which it can
activate a new row from the same bank.}
%
% To \hht{open a row in a bank that already has another row open,} the MC first
% precharges \hht{the bank (i.e., closes the open row)} by issuing a \cmdpre{}
% command. 
The \bgyellow{time interval for issuing a \cmdpre{} after an \cmdact{} must be} at
least \emph{restoration latency} (\tras{}). A DRAM chip performs a precharge
operation in two steps. First, the DRAM chip disables the wordline of the
activated row to disconnect its cells from the bitlines, and thus the row
buffer. Second, the precharge circuitry, which is part of a sense amplifier,
precharges the bitline to prepare it for the next row activation. The MC
\hht{follows} a \cmdpre{} with \hht{an} \cmdact{} to activate a new row at least
after the \emph{precharge latency} (\trp{}).

% Explain REF commands and how DRAM chips performs refresh
% Explain the refresh counter etc.
\subsection{Periodic DRAM Refresh}
\label{subsec:periodic_dram_refresh}
% \vspace{-10pt}

A DRAM cell capacitor loses its charge over time~\cite{liu2013experimental,
liu2012raidr, saino2000impact}, and losing too much charge results in a bit flip. The
\emph{retention time} of a cell refers to the duration for which its capacitor
stores the correct value. Cells in a DRAM chip have different retention times,
ranging from milliseconds to several hours~\cite{hassan2017softmc, kang2014co,
khan2014efficacy, kim2009new, lee2015adaptive, li2011dram, liu2013experimental,
liu2012raidr, patel2017reaper, qureshi2015avatar, venkatesan2006retention}. However, to
ensure data integrity, all \hht{DRAM cells} are uniformly refreshed at fixed
time intervals (typically 64, 32\hht{, or even \SI{16}{\milli\second}}), called
\emph{refresh window} (\trefw{}). To perform periodic DRAM refresh, the MC
issues a \cmdrefresh{} command at a fixed interval, denoted as \emph{refresh
interval} (\trefi{}) (typically 7.8 or \SI{3.9}{\micro\second}). A DRAM chip
refreshes several (e.g., $16$) rows upon receiving a single \cmdrefresh{}
command, and typically $8192$ \cmdrefresh{} commands refresh the entire DRAM
chip in a refresh window.

==> mainmatter/smd/sections/9_conclusion.tex <==
% \vspace{-5pt}
\section{Conclusion}
\label{sec:conclusion}
% \vspace{-10pt}

\hht{To set the memory controller free from managing DRAM maintenance
operations, \mechlong{} (\mech{}) introduces minimal changes to the existing
DRAM chips and memory controllers.} \mech{} enables in-DRAM maintenance
operations with no further changes to the DRAM interface, memory controller, or
other system components. Using \mech{}, we implement efficient maintenance
mechanisms for DRAM refresh, RowHammer protection, and memory scrubbing. \hhf{We show that these mechanisms altogether enable a higher performance, more energy efficient and at the same time more reliable and secure DRAM system.}
% To demonstrate the versatility of \mech{}, we implement two different
% maintenance mechanisms that perform periodic DRAM refresh, two different
% maintenance mechanisms that protect against RowHammer, and a maintenance
% mechanisms that perform memory scrubbing. In addition, we discuss other use
% cases that \mech{} enables. In our evaluation, we show that the maintenance
% mechanisms we implement using \mech{} significantly lower the performance and
% energy overhead compared to performing the same maintenance operations on
% existing DRAM chips. 
% We hope \mech{} inspires the researchers to develop new DRAM maintenance
% mechanisms that further reduce the overhead of maintenance operations and fix
% newly discovered reliability and security issues in DRAM. 
We believe \hhf{and hope that} \mech{} will enable practical adoption of
innovative ideas in DRAM design.  

==> mainmatter/softmc/abstract.tex <==
% !TEX root=../main.tex

\begin{abstract}
%DRAM, which stores data as charge in a capacitor, cannot retain 
%its data permanently,  as charge in the capacitor gradually leaks
%over time. The amount of charge in a cell impacts 
%how long a cell can retain data and how fast that cell can be read. 
%Continued scaling of DRAM process technology is making the cells smaller
%at each successive node.
%As a result, it is getting  difficult to store enough charge in
% smaller cell area, which directly impacts the retention, reliability, 
% and latency of DRAM cells.


DRAM is \revcrb{the primary technology} used for main memory in modern
systems. Unfortunately, as DRAM scales down to smaller technology
nodes, it faces key challenges in both \revcro{data integrity and latency},
which strongly affects overall system \revcrb{reliability and performance}.
To develop \revcrb{reliable and high-performance} DRAM-based main memory
in future systems, it is critical to characterize, understand, and
analyze various aspects \revcrb{(e.g., \revcro{reliability}, latency)}
of \revcrb{existing} DRAM chips. To enable this, there is a strong need for a
publicly-available DRAM testing infrastructure that can flexibly and
efficiently test DRAM chips in a manner accessible to both
software and hardware developers.
 
This paper develops the first such infrastructure, {\em SoftMC (Soft
  Memory Controller)}, an FPGA-based testing platform that
can control and test memory modules designed for the
commonly-used DDR (Double Data Rate) interface. SoftMC
has two key properties: {\em (i)} it provides {\em flexibility} to
thoroughly control memory behavior or to implement \revcrb{a wide range of}
mechanisms using DDR commands; and {\em (ii)} it is {\em easy to use}
as it provides a simple and intuitive high-level programming interface
for users, completely hiding the low-level details of the FPGA.

We demonstrate the capability, flexibility, and programming ease of SoftMC
with two example use cases. \revcrb{First}, we implement a test that
characterizes the retention time of DRAM cells. \revcrg{Experimental} results
we \revcrg{obtain} using SoftMC are consistent with the findings of prior
studies on retention time in modern DRAM, \revcrg{which serves} as a validation of our
infrastructure. \revcrb{Second, we} \revcrg{validate} two
recently-proposed mechanisms,
\revcrb{
\revcrg{which rely on accessing} recently-refreshed or recently-accessed DRAM cells
faster than other DRAM cells. % Although the hypothesis can be correct,
Using our infrastructure, we show that \revcrg{the expected latency
reduction effect of these mechanisms} is not observable in
existing DRAM chips,% we tested,
%The results generated using SoftMC on 24
%real DRAM chips do not show any evidence for this hypothesis, 
}%
 {} \revcrg{which demonstrates}
the usefulness of SoftMC in \revcro{testing} new ideas on
\revcrb{existing} memory
modules.  We discuss several other use cases of SoftMC, including the
ability to characterize emerging non-volatile memory modules that obey the
DDR standard. We hope that our open-source release of SoftMC fills a gap in
the space of publicly-available experimental memory testing infrastructures
and inspires new studies, ideas, and methodologies in memory system design.



%impacts makes it difficult to 
 
%%%successive generations, a number of important challenges have emerged that need to be
%%%addressed. First, even with continued process scaling, D

%%%Contiguous shrinking in process technology feature size makes DRAM cells more
%%%susceptible to errors. While the probability of occurrence of the already known
%%%reliability issues increases, previously unknown or not observable problems,
%%%such as Row-hammer, also emerge.
%%%
%%%We propose SoftMC, a FPGA-based memory controller for practical DRAM testing. SoftMC
%%%provides flexibility to implement the entire memory controller logic in
%%%software. Such design has the opportunity of practically running custom test
%%%algorithms to study new reliability issues and validate ideas from prior work.
%%%We implement two use cases with SoftMC to show its capabilities and limitations.
%%%The first use case runs a simple retention test on the DRAM module, whereas the
%%%second one evaluates an idea from prior work that states highly charged DRAM
%%%cells can be accessed with lower latency.  We provide a prototype implementation
%%%of SoftMC as a open-source software.
%%%

\end{abstract}


==> mainmatter/softmc/acknowledgements.tex <==
\vspace{-.05in}
\section*{Acknowledgments}
\label{section:acknowledgements}
\vspace{-.06in}
We thank the reviewers, the SAFARI group members, \revcrb{and Shigeki
Tomishima from Intel} for their feedback. We acknowledge the generous
support of Google, Intel, Nvidia, Samsung, and VMware. This work is
supported in part by NSF grants 1212962, 1320531, and 1409723, \revcro{the} Intel Science
and Technology Center for Cloud Computing, and the Semiconductor Research
Corporation.

\vspace{-.05in}


==> mainmatter/softmc/background.tex <==
\section{Background} 
\label{softmc_sec:background}

In this section, we first provide the necessary basics on DRAM organization and
operation. We also provide background on the DDR command interface, which is the
major standard for modern DRAM-based memories. For a more detailed description
of DRAM operation, we refer the reader to~\cite{kim2012case, liu2012raidr,
lee2013tiered, lee2015adaptive, chang2016understanding}.

\subsection{DRAM Organization}
\label{softmc_sec:dram_org}

Figure~\ref{softmc_fig:system_org} shows the organization of a DRAM-based memory
system. This system consists of \emph{memory channels} that connect the
processor to the memory. A channel has one or more \emph{ranks} that share the
control and data bus of the channel. A rank typically consists of multiple
(typically four to eight) DRAM chips. All DRAM chips in a rank share the command
signals such that they operate in lockstep. Each chip has an 8- or 16-bit wide
IO bus that contributes to the 64-bit IO bus of the channel. For example, four
DRAM chips (with a 16-bit IO bus per chip) are used to build the 64-bit IO bus
in the memory channel.

\input{mainmatter/softmc/figures/dram}

Figure~\ref{softmc_fig:chip_org} depicts a DRAM chip consisting of multiple
\emph{banks}. Each bank's cells can be accessed independently of other banks.
Figure~\ref{softmc_fig:bank_org} shows the key details of a bank, which consists of
\emph{(i)} a 2D cell array, \emph{(ii)} a row decoder, and \emph{(iii)} sense
amplifiers. A row of cells is connected to the row decoder through a wire called
\emph{wordline}, and a column of cells is connected to a sense amplifier through
a wire called \emph{bitline}. When accessing a row of cells, one of the
wordlines in the cell array is selected by the row decoder. Then, the
corresponding wordline driver raises the wordline, making electrical connections
between cells in the row and sense amplifiers through the bitlines. This
operation, i.e., accessing a row of cells, is referred to as row
\emph{activation}.

\subsection{DRAM Operations and Commands} 
\label{softmc_sec:dram_ops}

There are four DRAM operations necessary for data access and retention. We
describe them and their associated commands and timing constraints, as specified
in the DDR standard~\cite{jedec2008ddr3}.

   
\textbf{Activation.} When the memory controller receives a request to a row that
	is not already activated, it issues an \cmdact command with a row address to
	the DRAM. Then, the row decoder determines the wordline that corresponds to
	the requested row address, and enables that wordline to activate the cells
	connected to it. The activated cells share their charge with the bitlines
	that they are connected to. Then, sense amplifiers detect data by observing
	the perturbation that charge sharing created on the bitlines, and fully
	\emph{restore} the charge of the activated cells. At the end of activation,
	sense amplifiers contain the data of the activated row.


\textbf{Read/Write.} Some time after issuing the \cmdact command, the memory
	controller issues a column command, i.e., \cmdread or \cmdwrite, to select a
	portion of data in the activated row which corresponds to the requested
	column address. The \trcd timing parameter restricts the minimum time
	interval between an \cmdact command and a column command, to guarantee that
	the DRAM chip is ready to transfer data from the sense amplifiers to the
	memory channel. When the controller performs a \cmdread operation after any
	\cmdwrite command is issued to an open row in any bank, the \twtr timing
	parameter needs to be obeyed. Likewise, when the controller performs a
	\cmdwrite operation after any \cmdread command is issued to an open row in
	any bank, it needs to obey the \trtw timing parameter. During \twtr and
	\trtw, the DDR bus is switched between read and write modes, which is called
	bus turnaround.

\textbf{Precharge.} If a request to access a new row arrives while another row
	is currently activated in the same bank, the memory controller first needs
	to prepare the DRAM bank for the new row access.  This operation is called
	\emph{precharge}, and consists of two steps. First, the activated row in the
	bank needs to be \emph{deactivated}, by disconnecting and isolating the
	activated cells. Second, the sense amplifiers (and corresponding bitlines)
	need to be prepared (i.e., charged to the appropriate voltage levels) to
	detect data during the next row activation~\cite{lee2013tiered,
	lee2015adaptive}. There are three timing parameters related to the precharge
	operation. First, \tras{} specifies the minimum time interval between an
	\cmdact command and a \cmdprech command, to ensure that the activated cells
	are fully restored. Second, \twr {} (i.e., \emph{write recovery time})
	specifies the minimum time interval between the end of data transfer caused
	by a write command and a \cmdprech command, to ensure that the cells updated
	by the write operation are fully restored. Third, \trp{} specifies the
	minimum time between a \cmdprech command and an \cmdact command, to ensure
	that the precharge operation completes before the next activation.

\textbf{Refresh.} 
	A DRAM cell cannot retain its data permanently due to charge leakage. To
	ensure data integrity, the charge of the DRAM cell needs to be
	\emph{refreshed} (i.e., replenished) periodically. The memory controller
	replenishes cell charge by refreshing each DRAM row periodically (typically
	every \SI{64}{\milli\second}). The refresh period is specified by a timing
	parameter \trefi. The refresh operation can be performed at the rank or bank
	granularity~\cite{chang2014improving} depending on the DDR standard. Prior
	to issuing a \cmdrefresh command to a rank/bank, the memory controller first
	precharges all activated rows in the DRAM rank or the activated row in the
	DRAM bank that the refresh operation will be performed on. \trp{} specifies
	the minimum timing interval between a \cmdprech command and a \cmdrefresh
	command. After \trp, the memory controller issues a \cmdrefresh command to
	perform the refresh operation, which delays the subsequent \cmdact command
	to the refreshing rank/bank for an interval specified by \trfc. 

\subsubsection{DDR Command Interface} 
\label{softmc_sec:dram_cmd}

DDR commands are transmitted from the memory controller to the DRAM module
across a memory bus. On the memory bus, each command is encoded using five
output signals (\cmdcke, \cmdcs, \cmdras, \cmdcas, and \cmdwe).
Enabling/disabling these signals corresponds to specific commands (as specified
by the DDR standard).  First, the \cmdcke signal (\emph{clock enable})
determines whether the DRAM is in ``standby mode'' (ready to be accessed) or
``power-down mode''. Second, the \cmdcs (\emph{chip selection}) signal specifies
the rank that should receive the issued command.  Third, the \cmdras (\emph{row
address strobe})/\cmdcas (\emph{column address strobe}) signal  is used to
generate commands related to DRAM row/column operations. Fourth, the \cmdwe
signal (\emph{write enable}) in combination with \cmdras and \cmdcas, generates
the specific row/column command. For example, enabling \cmdcas and \cmdwe
together generates a \cmdwrite command, while enabling only \cmdcas indicates a
\cmdread command. 

So far, we have described the major DRAM operations and commands specified by
the DDR interface. Next, we motivate the need for a DRAM testing infrastructure
that can flexibly issue these DRAM commands via a high-level user interface.

==> mainmatter/softmc/figures/dram.tex <==
\begin{figure}[h]
	\centering
	\subfloat[System] {
		\includegraphics[height=0.9in]{figures/system}
		\label{softmc_fig:system_org}
	}
	\subfloat[Chip] {
		\includegraphics[height=0.9in]{figures/chip}
		\label{softmc_fig:chip_org}
	}
	\subfloat[Bank] {
		\includegraphics[height=0.9in]{figures/bank}
		\label{softmc_fig:bank_org}
	}
	\caption{DRAM-based memory system organization}
	\label{softmc_fig:dram_org}
\end{figure}


==> mainmatter/softmc/introduction.tex <==
% !TEX root=../main.tex

\section{Introduction}

DRAM (Dynamic Random Access Memory) is the predominant technology used
to build main memory systems of modern computers. The continued
scaling of DRAM process technology has enabled tremendous growth in
DRAM density in the last few decades, leading to higher capacity
main memories. Unfortunately, as the process technology node scales down to
the sub-\SI{20}{\nano\meter} feature size range, DRAM technology faces key challenges
that critically impact its \revcrb{reliability and performance}.

The fundamental challenge with scaling DRAM cells into smaller
technology nodes arises from the way DRAM stores data in cells. A DRAM
cell consists of a transistor and a capacitor. Data is stored as
charge in the capacitor. A DRAM cell cannot retain its data
permanently as this capacitor leaks its charge gradually over
time. 
%The time a cell can retain its data is called the retention time
%of the cell. 
To maintain correct data in DRAM, each cell is
periodically refreshed to replenish the charge in the capacitor. 
\revcrb{At smaller technology nodes,} it is becoming increasingly
difficult to store \revcrb{and retain} enough charge in a cell,
\revcrb{causing various reliability \revcro{and performance} issues}\revcrg{~\cite{liu2012raidr, liu2013experimental}}. 
\revcrb{Ensuring reliable operation of the DRAM cells is a key challenge in
future technology nodes}~\cite{mutlu2013memory, mandelman2002challenges,
  kim2005technology, mueller2005challenges, liu2012raidr,
  kang-memcon2014, liu2013experimental}.

The fundamental problem of retaining data with less charge in smaller
cells directly impacts the \revcrb{reliability and
performance} of DRAM
cells. First, smaller cells placed in close proximity make cells more
susceptible to various types of interference. This potentially
disrupts DRAM operation by flipping bits in DRAM, resulting in major
reliability issues~\cite{kim2014flipping, nakagome1988impact,
  redeker2002investigation, schroeder2009dram, sridharan2013feng,
  meza-dsn2015}, which can lead to system
failure~\cite{schroeder2009dram,meza-dsn2015} or security
breaches~\cite{kim2014flipping, seaborn2015exploiting, seaborn2015exploiting2, rowhammerjava2015,
van2016drammer, xiao2016one, razavi2016flip}.  Second, it takes longer time
to access a cell with less charge~\cite{hassan2016chargecache,
lee-hpca2015}, \revcrb{and write latency increases as the access transistor size
reduces~\cite{kang-memcon2014}}. \revcro{Thus}, smaller cells directly
impact DRAM latency, as DRAM access latency is determined by the worst-case
(i.e., {\em slowest}) cell in any chip~\cite{chandrasekar2014exploiting,
lee-hpca2015}. DRAM access latency has not improved with
technology scaling in the past decade~\cite{lee-hpca2013, jung-2005,
borkar-cacm2011, mutlu2013memory}, and, in fact, some latencies
are expected to increase~\cite{kang-memcon2014}, making memory latency an
increasingly critical system performance bottleneck.

As such, there is a significant need for new mechanisms that improve
the reliability and performance of DRAM-based main memory systems. In
order to design, evaluate, and validate many such mechanisms, it is
important to accurately characterize, analyze, and understand
DRAM (cell) behavior in terms of \revcrb{reliability and latency}. For such
an understanding to be accurate, it is critical that the characterization
and analysis be based on the \revcrb{\emph{experimental} studies} of {\em
real DRAM chips}, since a large number of factors (e.g., various types of
cell-to-cell interference~\cite{nakagome1988impact,
redeker2002investigation, kim2014flipping}, inter\revcrb{-} and intra-die process
variation~\cite{chang2016understanding, lee2016reducing, nassif2000delay,
chandrasekar2014exploiting, lee-hpca2015}, random effects~\cite{liu2013experimental,
yaney1987meta, srinivasan1994accurate, hazucha2000impact}, operating
conditions~\cite{liu2013experimental, lee2010mechanism}, internal
organization~\cite{liu2013experimental, hidaka1989twisted, khan2016parbor}\revcrb{, stored
data patterns~\cite{khan2016case, khan2016parbor, liu2013experimental}})
concurrently impact the \revcrb{reliability and latency} of cells. Many of
these phenomena and their interactions cannot be properly modeled (e.g., in
simulation or using analytical methods) without rigorous experimental
characterization and analysis of real DRAM chips.  The need for such
experimental characterization and analysis, with the goal of building the
understanding necessary to improve \revcrg{the} {}\revcrb{reliability and performance} of
future DRAM-based main memories at various levels (both software and
hardware)\revcrb{,} motivates the need for a publicly-available DRAM
testing infrastructure that can enable system users and designers to
characterize real DRAM chips.

Two key features are desirable from such an experimental memory
testing infrastructure.  \rev{First, the infrastructure should be {\em
flexible} enough to test any DRAM operation (supported by the
commonly-used DRAM interfaces, e.g., the standard Double Data Rate, or DDR,
interface) to characterize cell behavior or evaluate the impact of a
mechanism (e.g., adopting different refresh rates for different 
cells~\cite{liu2012raidr, venkatesan2006retention, khan-sigmetrics2014, 
qureshi-dsn2015, khan2016case}) on real DRAM chips.}
% Two key features are desirable from such an experimental memory
% testing infrastructure.  First, the infrastructure should be {\em
%   flexible} enough to test any DRAM operation (supported by the
% commonly-used DRAM interfaces, e.g., the standard Double Data Rate, or DDR, 
% interface) to characterize cell behavior or evaluate the impact of a
% mechanism that uses such operations.  For example, in order to
% characterize the retention time of cells in modern DRAM chips, we need
% a platform that can issue refresh operations to DRAM at different time
% intervals under varying operating conditions (e.g., different data
% patterns).  Similarly, the reliability guarantees of a mechanism that
% improves DRAM energy efficiency and performance, by adopting different
% refresh rates for different cells~\cite{liu2012raidr,
%   venkatesan2006retention, khan-sigmetrics2014, qureshi-dsn2015}, can
% be characterized on real chips by implementing this mechanism (i.e.,
% various refresh rates that are customized for different cells) in the testing
% infrastructure.  
Second, the infrastructure should be {\em easy to
  use}, such that it is possible for both software and hardware
developers to implement new tests or mechanisms without \revcrg{spending}
significant time and effort.  For example, a testing infrastructure
that requires circuit-level implementation, detailed knowledge of the
physical implementation of DRAM data transfer protocols over the
memory channel, or low-level FPGA-programming to modify the
infrastructure would severely limit the usability of such a platform
to a limited number of experts.


This paper designs, prototypes, and demonstrates the basic
capabilities of \revcrb{such} a flexible and easy-to-use experimental DRAM
testing infrastructure, called {\em SoftMC (Soft Memory
  Controller)}. SoftMC is an open-source FPGA-based DRAM testing infrastructure,
consisting of a programmable memory controller that can control and
test memory modules designed for the commonly-used DDR (Double Data
Rate) interface. To this end, SoftMC implements {\em all}
low-level DRAM operations (i.e., DDR commands) available in a typical
memory controller (e.g., opening a row in a bank, reading a specific
column address, performing a refresh operation, enforcing various
timing \revcrb{constraints} between commands). 
\rev{Using these low-level operations, SoftMC can test and characterize any
(existing or new) DRAM mechanism \revcrb{that uses the existing DDR
interface}.  SoftMC provides a
%   flexibility} to thoroughly control any aspect of memory behavior using
%   these low-level DRAM operations. It can test and characterize
% any (existing or new) mechanism comprised of these low-level
% operations. SoftMC is {\em easy to program}: it provides a
simple and intuitive high-level programming interface 
that completely hides the low-level details of the FPGA from 
users.} Users implement their \revcro{test} routines or mechanisms in a
high-level language that \revcrb{automatically} gets translated into the
low-level SoftMC memory controller operations in the FPGA.

%We provide a prototype implementation of SoftMC on the widely used
%Xilinx ML605 FPGA board~\cite{ml605}. Our implementation has three
%major components: {\em (i)} A C/C++ API that provides the users with
%all DDR commands along with the flexibility to adjust the timing
%between these commands. Using these commands, it is possible to test
%one specific operation (e.g., refresh or activation) or implement any
%algorithm using a combination of the commands (e.g., hammering one
%specific row by continuously accessing it~\cite{kim2014flipping} or
%using different refresh intervals for different regions of the DRAM
%chip~\cite{liu2012raidr, liu2013experimental, khan-sigmetrics2014,
%  qureshi-dsn2015}). Users write programs using only this C/C++ API to
%to implement their tests or mechanisms. {\em (ii)} A driver that sends
%the DRAM commands to the FPGA board using the PCIe bus.  {\em (iii)} A
%low-level implementation of these DRAM commands on the FPGA using
%register transfer language (Verilog). This low-level implementation is
%the memory controller, which interfaces with the DRAM chips over the
%bus, and is not exposed to the users of the infrastructure.

 
%%% ONUR: Do we analyze the impact of different operating conditions
%%% in the retention time test? (See below). If not, we should remove
%%% that phrase.
%%% ONUR: Based on the current results, I removed this:
% and analyze the impact of different operating conditions (e.g., data
% pattern, temperature) on retention time of cells.

\rev{SoftMC can be used to implement any DRAM test or mechanism
consisting of DDR commands, without requiring significant effort.
Users can verify whether the test or mechanism works successfully
on real DRAM chips by monitoring whether any errors are
introduced into the data.  The high-level programming interface
provides simple routines to verify data integrity at any point
during the test.  SoftMC offers a wide range of use cases, such
as characterizing the effects of variation within \revcro{a DRAM chip} and across
DRAM \revcro{chips}, verifying the correctness of new DRAM mechanisms on actual
hardware, and experimentally discovering the \revcrb{reliability, retention, and
timing} {}\revcrg{characteristics} of an unknown or newly-designed
DRAM chip \revh{(or finding the best specifications for a known DRAM
chip)}. We demonstrate the potential and ease of \revcrb{use of} SoftMC by
implementing two use cases.}

% SoftMC can be used to implement any DRAM test or mechanism consisting
% of DDR commands, without requiring significant effort. We demonstrate
% the capability, flexibility, and programming ease of SoftMC by
% implementing two use cases.  
First, we demonstrate the ease of use of
SoftMC's high-level interface by implementing a simple retention time
test. Using this test, we characterize the retention time \revcro{behavior}
of cells in modern DRAM chips.  Our test results match the prior
experimental studies that characterize DRAM retention time in modern
DRAM chips~\cite{liu2012raidr, liu2013experimental, khan-sigmetrics2014,
qureshi-dsn2015}, providing a validation of our infrastructure.

Second, we demonstrate the flexibility and capability
of SoftMC by validating \revcrb{two} recently-proposed DRAM latency
reduction mechanisms~\cite{hassan2016chargecache, shin2014nuat}. These
mechanisms exploit the \revcrg{idea} that highly-charged DRAM cells can be
accessed with low latency. DRAM cells \revcrg{are} in a highly-charged state when
they are recently refreshed or recently accessed.  Our SoftMC-based
experimental analysis of 24 real DRAM chips from three major DRAM vendors
\revcrb{demonstrates that the expected \revcrg{latency reduction} effect of these mechanisms is
\emph{not} observable in existing DRAM chips.
% does {\em not} provide \revcrb{evidence that their hypothesis affects the
% existing DRAM chips.  
We discuss the details of our experiments
% and discussion about why the highly-charged cells cannot be accessed fast in
% existing DRAM chips 
in Section~\ref{sec:nuat_test} {}\revcrg{and provide reasons as to why the
effect is not observable in existing chips.}}
%evidence for the hypothesis that highly-charged cells can be accessed
%faster than other cells. We believe the reason is that
%charge does not leak fast enough from the DRAM cells to provide any
%significant variation in cell access latency. 
This experiment demonstrates {\em (i)} the
importance of experimentally characterizing real DRAM chips to understand the
behavior of DRAM cells, and designing mechanisms that are based on this
experimental understanding; and {\em (ii)} the effectiveness of SoftMC in testing
(validating or refuting) new ideas on \revcrg{existing} memory modules.



%We believe that the reason is the large margin on the latency in
%modern DRAM chips to provide reliability against random failures and
%the worst-case operating conditions. Due to this large margin, the
%amount of charge does not significantly change over time within 64ms,
%making the cell access latency insensitive to refresh. This experiment
%demonstrates {\em (i)} the importance of experimentally characterizing
%real DRAM chips to understand the behavior of DRAM cells and designing
%mechanisms that are based on this experimental understanding, {\em
%  (ii)} the effectiveness of SoftMC in testing (validating or
%refuting) new ideas on real memory modules.

% \rev{Another use case is that SoftMC can be used to identify timing, retention,
% and reliability specifications of an unknown DRAM chip, i.e., newly manufactured
% chip.} 
We also discuss several other use cases of SoftMC, including the ability
to characterize emerging non-volatile memory modules that obey the DDR standard.
We hope that SoftMC inspires other new studies, ideas, and methodologies in
memory system design.

%%% ONUR Modified until here

This work makes the following major contributions:

\squishlist

\item We introduce SoftMC, \revcrb{the first} open-source
  \revcrb{FPGA-based} experimental memory 
  testing infrastructure. SoftMC implements all low-level DRAM operations in a
  programmable memory controller that is exposed to the user with a
  flexible and easy-to-use interface, and hence enables the efficient
  characterization of modern DRAM chips and evaluation of mechanisms
  built on top of low-level DRAM operations. To our knowledge, SoftMC
  is the first publicly-available infrastructure that exposes a
  high-level programming interface to ease memory testing and
  characterization.

\item We provide a prototype implementation of SoftMC with a
  high-level software interface for users and a low-level FPGA-based
  implementation of the memory controller. We have released the
  software interface and the implementation publicly as a
  freely-available open-source tool~\cite{safarigithub}.

\item We demonstrate the capability, flexibility, and programming ease
  of SoftMC by implementing two example use cases. Our second use case
  demonstrates the effectiveness of SoftMC as a new tool to \revcro{test
  existing} or new mechanisms \revcro{on existing memory chips}. Using SoftMC, we
  demonstrate \revcrb{that the expected effect (i.e., highly-charged DRAM
  rows can be accessed faster than others) of} two recently-proposed
  mechanisms \revcrb{is not observable} in 24 modern DRAM chips from three major
  manufacturers.
\squishend





%********************************************
%%%Due to its low cost-per-bit, Dynamic Random Access Memory (DRAM) is widely used
%%%to architect main memory subsystems today. While the continued scaling of the
%%%process technology has enabled lower cost-per-bit and higher integration over
%%%successive generations, a number of important challenges have emerged that need to be
%%%addressed. First, even with continued process scaling, DRAM access latency has
%%%remained almost constant, making memory latency a critical performance bottleneck in
%%%today's systems. Second, DRAM cells are composed of a single transistor and capacitor pair
%%%which stores one bit of information. Although such a design allows high capacity
%%%due to small area requirements, the
%%%capacitor gradually leaks charge over time which causes the data to be lost
%%%after a certain period. To maintain the correct data, the charge in the
%%%capacitors need to be replenished using periodic refresh operations.
%%%The duration in which a DRAM cell is able to contain the data is called
%%%retention time. With the scaling of the process technology, achieving high retention times and
%%%ensuring reliable DRAM operation are becoming more
%%%difficult~\cite{mutlu2013memory,mandelman2002challenges,kim2005technology,mueller2005challenges}.
%%%Third, increasing cell density has a negative impact on cell reliability making
%%%reliability of DRAM chips a key concern.
%%%For example, placing cells closer to each other makes the cells more susceptible
%%%to disturbance errors. Recently,
%%%Kim et al~\cite{kim2014flipping} introduced the Row-hammer phenomenon which causes
%%%faster charge leakage in DRAM cells due to excessive accesses to nearby cells.
%%%
%%%
%%%To address these growing issues, performing extensive performance and reliability
%%%characterization of the DRAM chips is of vital importance. 
%%%In order to understand DRAM performance and reliability at the low level (for
%%%example, testing retention time under different operation conditions), we
%%%need a flexible and easy-to-use test infrastructure. To effectively
%%%perform this characterization, two key features are desirable from the test
%%%infrastructure. First, such a 
%%%system should be easily modifiable to evaluate prospective problems with low
%%%effort and cost. Second, the infrastructure should be flexible enough to
%%%perform a wide range of tests to effectively characterize DRAM.
%%%
%%%
%%%The approaches introduced in prior work are not sufficent to address the
%%%practicality and flexibility features.  Prior studies mainly focuses on
%%%approaches that we can separate into two categories. First, many studies propose
%%%Built-in Self Test (BIST) architectures where DRAM chips include a special logic
%%%which performs the tests.  The advantage of the BIST architecture is that they
%%%can achieve low testing times compared to other approaches~\cite{yang2015hybrid,
%%%bernardi2010programmable, querbach2014reusable}.  However, these mechanisms
%%%mostly consist of hard-coded circuits which can evaluate only pre-defined test
%%%cases. Adapting BIST for new test cases requires new hardware design and
%%%re-manufacturing of the chip which imposes high cost. In the second category,
%%%prior work propose Automatic Testing Equipment (ATE). Although such approaches
%%%provide better flexibility, they are still have important limitations. Huang et
%%%al.~\cite{huang2000fpga} proposed an FPGA-based reconfigurable DRAM tester.
%%%Their scheme is limited to testing only different data patterns using several
%%%pre-defined test algorithms. Another approach provides better programmability
%%%but requires special equipment to conduct the tests~\cite{yang2015random}.
%%%
%%%
%%%
%%%In this work, we introduce a new FPGA-based DRAM testing infrastructure which
%%%targets testing DDR-based memory modules. The infrastructure consists of an FPGA
%%%which is programmed to run our memory controller design called SoftMC. 
%%%SoftMC only implements the DDR physical layer (rather than a fixed memory
%%%controller design) and exposes different low-level DDR
%%%commands. As a result, the infrastructure provides the flexibility to implement
%%%\emph{any} memory controller logic or DRAM test program. At the same time, SoftMC is
%%%programmable using a high-level language with simple APIs, making the
%%%infrastructure easy to use, reducing programmer effort and time.
%%%
%%%SoftMC comprises several hardware and software components to interface between
%%%the host machine and the DRAM under test. A key component is the FPGA which can
%%%be programmed to implement the logic for different memory controller designs and
%%%to generate low-level DDR commands. The SoftMC driver, which runs on the host
%%%machine, provides an interface to the host machine for low-level control over
%%%the DRAM. Using this interface, the user can implement different DRAM tests and
%%%memory controller designs from the host machine entirely in software using a
%%%high-level language. We provide simple APIs in C++ to enable the user to quickly
%%%implement any memory controller logic and generate low-level DRAM commands using
%%%SoftMC instructions. The communication
%%%between the FPGA and the host machine is handled via high-speed PCI Express 2.0
%%%interface~\cite{budruk2004pci}. 
%%%
%%%
%%%SoftMC is practical to use because it is FPGA-based and does not require any hardware
%%%modifications to implement different memory controller designs. We provide a
%%%prototype implementation of SoftMC on widely used Xilinx ML605 FPGA board~\cite{ml605}.
%%%Any user who wants to test DRAM under various conditions can set up his/her
%%%infrastructure practically at low cost. Implementing custom test programs would
%%%take a negligible amount of time as we provide a simple C++ API to work with. SoftMC provides
%%%sufficient flexibility to implement a wide set of memory controller logic by
%%%exposing the entire list of DDR commands given in the specification to the
%%%software. We designed SoftMC with the intention to use it to validate ideas about DRAM
%%%practically and quickly. Therefore, SoftMC sacrifices performance for
%%%flexibility.
%%%
%%%
%%%In Section~\ref{sec:use_cases}, we provide two use cases to
%%%demonstrate the capabilities and the limitations of our design. As a first use
%%%case, we show how to implement a simple retention time test. We believe that the
%%%retention time test provides some insight about the practicality of the SoftMC.
%%%Second, we evaluate an idea from prior work. Shin et al.~\cite{shin2014nuat}
%%%experimentally show that recently refreshed DRAM cells which contain higher
%%%amount of charge compared to less recently refreshed cells can be accessed with
%%%lower latency. We show how to evaluate this idea using SoftMC and provide
%%%results obtained from three DDR3 modules from three different vendors. We do
%%%not observe any results that support the experimental evaluation of Shin et al.
%%%
%%%In this work, we make the following contributions:
%%%
%%%\squishlist
%%%\item We introduce a new DRAM testing infrastructure, SoftMC, which is practical to use
%%%and provide flexibility to implement a wide range of test programs
%%%\item We provide a prototype implementation of SoftMC for widely used ML605
%%%board. We release that implementation as an open-source tool.
%%%\item We demonstrate how SoftMC works by two use cases. The first one is a
%%%simple retention test, where the second one evaluates a recently proposed
%%%idea.
%%%
%%%\squishend


==> mainmatter/u-trr/0_abstract.tex <==
\begin{abstract}

    The RowHammer vulnerability in DRAM is a critical threat to system security.
    To protect against RowHammer, vendors commit to security-through-obscurity:
    \hht{modern} DRAM \hhth{chips rely} on undocumented, proprietary, on-die
    mitigations, commonly known as \emph{Target Row Refresh} \hhn{(TRR)}.
    \hhth{At a high level, TRR detects and refreshes potential RowHammer-victim
    rows, but its exact implementations are not openly disclosed. Security
    guarantees of \hhn{TRR mechanisms} cannot be easily studied due to their
    proprietary nature.}

    To assess \hh{the} security guarantees of recent \hh{DRAM} \hhth{chips}, we
    present \emph{\hh{Uncovering} TRR} (\method{}), an experimental methodology
    to analyze \hht{in-DRAM} TRR implementations. \method{} is based on the \hhth{new}
    observation that \hht{data} retention failures in DRAM enable a side channel
    that leaks information on how TRR refreshes potential victim rows.
    % OPTIONAL: A VERY GOOD AND SUCCINT EXAMPLE HERE
    \method{} allows us to (i) understand how logical \hh{DRAM} rows are laid
    out physically in silicon; (ii) study undocumented on-die TRR
    \hh{mechanisms}; and (iii) combine (i) and (ii) to evaluate \hh{the}
    RowHammer security guarantees of modern DRAM \hht{chips}. We show how
    \method{} allows us to craft RowHammer access patterns that successfully
    circumvent \hhth{the TRR mechanisms \hhf{employed in \numTestedDIMMs{} DRAM
    modules} of the three major} DRAM vendors. We find that \hhe{the
    \hhf{DRAM} modules we} \hhf{analyze} are vulnerable to RowHammer\hht{,
    having} bit flips in up to \vulnRowsMaxPct{}\% of all DRAM rows.
    % OPTIONAL: ADD SOME WORDS ON HOW THIS IS SO MUCH BETTER THAN TRRESPASS

% 
%     The RowHammer vulnerability of modern DRAM is a critical threat to
%     system security. To protect against RowHammer, modern DRAM chips implement
%     Target Row Refresh (TRR).
%     % , whose key premise is to refresh the
%     % neighbor rows of a hammered row. The DRAM vendors follow this key premise to implement their TRR
%     % mechanisms but still the implementation
%     % details lead to differences in the protection guarantees of TRR against
%     % RowHammer. 
%     As of today, none of the three major DRAM vendors has released
%     the implementation details of their TRR designs, and therefore the
%     protection capabilities of the TRR mechanisms are not verified. In fact, a
%     recent prior work, TRRespass, unveils several high-level details of the
%     in-DRAM TRR mechanisms and proposes a fuzzing-based technique to generate
%     DRAM access patterns that bypass the TRR protection to cause
%     RowHammer bit flips. However, TRRespass does not provide sufficient insights
%     to fully understand different TRR implementations, assess their protection
%     capabilities, and craft a DRAM access pattern that precisely bypasses TRR.
%     
%     In this paper, we propose \hh{Unveiling TRR (\method{})}, an experimental
%     methodology to reverse-engineer the implementation of different TRR
%     mechanisms and gain insights to craft DRAM access patterns that precisely
%     \hh{and very efficiently} circumvent the TRR protection. \method{} is based
%     on a new technique that leverages the retention failures in a DRAM row to
%     gain visibility into how TRR refreshes potential victim rows. For example,
%     not having retention failures in row $R_0$, when accessing another row $R_1$
%     at half of the retention time of $R_0$, shows that TRR refreshes $R_0$ to
%     mitigate potential RowHammer bit flips. \hh{Our newly developed understanding enables us to craft access patterns that are greatly more effective in inducing RowHammer bit flips than state-of-the-art approaches, i.e., TRRespass.} Using \method{}, we unveil 1) the
%     aggressor-row-detection mechanism and 2) when TRR performs additional
%     refreshes. These insights help us craft a new DRAM access pattern that
%     successfully circumvents the TRR mechanism of one of the vendors. Our
%     analysis shows that all modules of the same vendor are vulnerable to the new
%     access pattern and up to \vulnRowsMaxPct{}\% of the all DRAM rows, on
%     average, get at least one bit flip when hammered.
% 
\end{abstract}


==> mainmatter/u-trr/1_intro.tex <==
% !TEX root=../main.tex

\vspace{-2mm}

\section{Introduction}
\label{sec:intro}
\vspace{-1mm}
% Hasan: The two paragraphs below are redundant as we explain the same in more detail in later paragraphs
% It is long understood that security cannot be achieved \hht{only} through
% obscurity~\hht{\cite{scarfone2008guide, anderson2020security,
% saltzer1975protection}}. \hht{Yet, such} is the current state of practice when
% it comes to DRAM, the most prevalent memory technology today. The DRAM
% technology suffers from bit flips caused through the RowHammer
% vulnerability~\hht{\cite{kim2014flipping, mutlu2019rowhammer}}. \hhth{The}
% \hht{main} mitigation \hht{mechanism} that is currently protecting systems
% against the plethora of known \hh{RowHammer}
% attacks~\hht{\cite{cojocar2019exploiting, gruss2018another, gruss2016rowhammer,
% lipp2018nethammer, qiao2016new, razavi2016flip, seaborn2015exploiting,
% tatar2018defeating, van2016drammer, xiao2016one, frigo2020trrespass,
% ji2019pinpoint, kwong2020rambleed, mutlu2017rowhammer, van2018guardion,
% kim2020revisitingrh, deridder2021smash, mutlu2019rowhammer, pessl2016drama,
% bosman2016dedup, bhattacharya2016curious, jang2017sgxbomb, aga2017good,
% frigo2018grand, hong2019terminal, cojocar2020we, weissman2020jackhammer,
% zhang2020pthammer, rowhammergithub, yao2020deephammer}} is the obscure,
% undocumented, and proprietary Target Row Refresh
% (TRR)\hht{~\cite{frigo2020trrespass}} deployed inside DRAM chips. 

% To show the flaw with this security-through-obscurity strategy, we \hht{first}
% present \method{}, a novel \hht{methodology} that uses retention failures as a
% side channel for precisely determining the operation of the in-DRAM TRR
% mechanisms in \hht{DRAM chips} from \hhth{all three major DRAM} vendors. Using
% the insights from \method{}, we craft specialized \hhth{access} patterns that
% bypass TRR on \hht{DRAM chips} from all three major vendors. Such insights are
% important to understand the weaknesses of the TRR implementations \hht{to
% develop 1)} more efficient RowHammer attacks \hht{and 2) truly-secure protection
% mechanisms against RowHammer}.

% \vspace{1mm} 
% DRAM and discovery of RowHammer as a disturbance error in DRAM
% \noindent \textbf{RowHammer attacks.} 
DRAM~\hhf{\cite{dennard1968field}} has long been the dominant memory technology
used in almost all computing systems due to its \hht{low latency and} low cost
per bit. DRAM vendors still push DRAM technology \hht{scaling} forward to
continuously shrink DRAM cells to further reduce the cost of
DRAM\hht{~\cite{mutlu2013memory}}. \hhth{Unfortunately, DRAM technology scaling
leads to increasingly important DRAM reliability problems as DRAM cells get
smaller and the distance between the cell reduce.} Kim et
al.~\cite{kim2014flipping} report that most DRAM \hht{chips} \hhth{manufactured
since 2010} are susceptible to disturbance errors \hhth{that are}
\hht{popularly} referred to as RowHammer. Recent works~\hht{\cite{yang2019trap,
walker2021dram, kim2014flipping, mutlu2019rowhammer, ryu2017overcoming,
park2016experiments, yang2016suppression, yang2017scanning, gautam2019row,
jiang2021quantifying}} explain the circuit-level
charge leakage mechanisms that lead to the RowHammer vulnerability. 
% A RowHammer attack can be performed by 
\hh{\hht{A security} attack exploits the RowHammer vulnerability by} hammering
(i.e., repeatedly activating and precharging) \hhf{an} \emph{aggressor} row
many times (e.g., \hhf{$139K$ in DDR3~\cite{kim2014flipping},} \hhth{$10K$ in
DDR4~\cite{kim2020revisitingrh}, and $4.8K$ in
LPDDR4~\cite{kim2020revisitingrh})}\footnote{\jk{For DDR3 chips,
\cite{kim2014flipping} reports the minimum number of row activations on a
\emph{single} aggressor row (i.e., single-sided RowHammer) to cause a RowHammer
bit flip. For DDR4 and LPDDR4 chips, \cite{kim2020revisitingrh} reports the
minimum number of row activations to \emph{each of the two}
immediately-adjacent aggressor rows (i.e., double-sided RowHammer).}}
%\footnote{\hhf{For DDR3 chips,
%\cite{kim2014flipping} reports the minimum row activation counts that are needed
%to cause a RowHammer bit flips by hammering a single aggressor row (i.e.,
%performing single-sided RowHammer). For DDR4 and LPDDR4 chips,
%\cite{kim2020revisitingrh} reports the same by hammering two aggressor rows
%(i.e., performing double-sided RowHammer).}}} 
to cause bit flips in the cells of the \emph{victim} rows that are
\hh{physically adjacent} to the hammered row. Since the discovery of RowHammer,
researchers \hht{have} proposed many techniques that take advantage of the
RowHammer vulnerability to \hht{compromise operating
systems~\cite{seaborn2015exploiting, van2018guardion, van2016drammer,
gruss2016rowhammer, cojocar2019exploiting, qiao2016new, kwong2020rambleed,
pessl2016drama, bhattacharya2016curious, jang2017sgxbomb, zhang2020pthammer,
cojocar2020we, weissman2020jackhammer, ji2019pinpoint}, web
browsers~\cite{gruss2018another, bosman2016dedup, frigo2020trrespass,
deridder2021smash, frigo2018grand}, cloud virtual machines~\cite{razavi2016flip,
xiao2016one}, remote servers~\cite{tatar2018defeating, lipp2018nethammer}, and
deep neural networks~\cite{yao2020deephammer,
hong2019terminal}.}\footnote{\hht{A review of many RowHammer attacks \hhf{and
defenses} is provided in~\cite{mutlu2019rowhammer}.}} \hhth{Thus}, RowHammer is
a \hhth{clear} major threat to \hh{system} security.


%The hammered row is
%typically referred to as the \emph{aggressor} and its neighbors as the \emph{victims}.

%Compared to hammering a single aggressor (single-sided RowHammer), prior
%works~\cite{kim2020revisitingrh, frigo2020trrespass, gruss2018another,
%seaborn2015exploiting, aweke2016anvil} show that hammering both neighbors of a
%victim row (double-sided RowHammer) at the same time leads to more bit flips
%and lower hammer counts to induce a bit flip.

%Prior
%works~\cite{cojocar2019exploiting, gruss2018another, gruss2016rowhammer,
%lipp2018nethammer, qiao2016new, razavi2016flip, seaborn2015exploiting,
%tatar2018defeating, van2016drammer, xiao2016one, frigo2020trrespass,
%ji2019pinpoint, kwong2020rambleed, mutlu2017rowhammer, van2018guardion,
%kim2020revisitingrh,deridder2021smash} show that RowHammer affects many systems since nearly all

% How a RowHammer attack is performed, double-sided RowHammer

% Security impact/implications of RowHammer

% Overview of TRR. Importance of REF commands and DRAM refresh
%\footnote{The memory controller must typically issue DRAM refresh
%commands at certain intervals to refresh each DRAM row once every $64ms$.
%However, operating at extended temperature ranges require refresh at 2x/4x
%rate~\cite{ddr4,ddr4operationhynix,2014lpddr4}} 

% \vspace{1mm}
% \noindent \textbf{Target Row Refresh.} 
To prevent RowHammer, DRAM vendors equip their DRAM \hht{chips} with a
\emph{mitigation mechanism} known as Target Row Refresh
(TRR)~\cite{frigo2020trrespass, cojocar2019exploiting,kim2020revisitingrh,
micronddr4trr}. The main idea \hht{of} TRR is to detect an aggressor row
\hht{(i.e., a row \hhth{that is being} rapidly activated)} and refresh its
\hhth{victim rows} \hht{(i.e., \hhf{neighboring rows that are} physically
adjacent to the aggressor row)}. \hhth{TRR} refreshes the victim rows
\hhth{separately from} the \emph{regular} refresh operations\hhf{~\cite{raidr,
venkatesan2006retention, liu2013experimental, cui2014dtail, bhati2015flexible}}
that must periodically \hhth{(e.g., once every \SI{64}{\milli\second})} refresh
each DRAM row in the entire DRAM \hht{chip}. Some of the major DRAM vendors
advertise \emph{RowHammer-free} DDR4 DRAM
\hht{chips}~\hht{\cite{samsung2014trrDram, micronddr4, frigo2020trrespass}}.
However, none of the DRAM vendors \hht{have so far} disclosed the implementation
details \hht{let alone} proved the protection guarantees of their TRR
mechanisms. \hhf{It is long understood that security cannot be achieved
\hht{only} through obscurity~\cite{scarfone2008guide, anderson2020security,
saltzer1975protection}. Yet, such is the current state of practice when it comes
to DRAM.}

The recent TRRespass work~\cite{frigo2020trrespass} shows that in certain DRAM
\hht{chips}, the TRR mechanism keeps track of \hht{only} a few \hhth{aggressor
rows}. \hht{Hence, an access pattern that hammers many aggressor rows can
circumvent the TRR protection and induce RowHammer bit
flips}.
% \footnote{\hht{TRRespass~\cite{frigo2020trrespass} proposes RowHammer
% access patterns that hammer many DRAM rows at the same time to exceed the number
% of rows that TRR can keep track of.}} 
While \hhn{TRRespass} already \hh{demonstrates
\hht{the flaws of}} certain TRR implementations, it does \emph{not} \hh{propose
a methodology for \emph{discovering} these \hht{flaws}}. \hh{\hht{According
to~\cite{frigo2020trrespass},} simply increasing the number of \hhth{aggressor
rows} is \emph{not} \hht{sufficient} to \hht{induce} bit flips on \hhth{29 out
of 42} of the DDR4 \hhth{modules that were tested by~\cite{frigo2020trrespass}}.
\hht{However,} it is unclear whether such DDR4 \hht{chips} are \emph{fully}
secure due to the lack of insight into the \hhn{detailed} operation of TRR in these
\hht{chips}.} \hhth{Thus, we need new methods for identifying whether or not
DRAM chips are fully secure against RowHammer.}

% Furthermore, simply increasing the number of aggressors is not enough to
% trigger bit flips on \hh{many of the} existing DDR4 devices. However, due to the
% lack of insight into the operation of TRR in these devices, it is not clear
% whether they are \hh{\emph{fully}} secure.

%use an FPGA-based
%infrastructure to gain some insights about the TRR mechanisms implemented
%inside DRAM to develop TRRespass, a testing tool that generates TRR-aware
%access patterns that could still induce RowHammer bit flips. The TRR-aware
%access patterns typically include many aggressor rows (up to 19), and therefore
%the authors refer to such access pattern as \emph{many-sided RowHammer}. They
%show that, despite being advertised as RowHammer-free, recent DDR4 and LPDDR4
%DRAM devices are still vulnerable to RowHammer.


%In a recent study, Frigo et al.~\cite{frigo2020trrespass} use an FPGA-based
%infrastructure to gain some insights about the TRR mechanisms implemented
%inside DRAM to develop TRRespass, a testing tool that generates TRR-aware
%access patterns that could still induce RowHammer bit flips. The TRR-aware
%access patterns typically include many aggressor rows (up to 19), and therefore
%the authors refer to such access pattern as \emph{many-sided RowHammer}. They
%show that, despite being advertised as RowHammer-free, recent DDR4 and LPDDR4
%DRAM devices are still vulnerable to RowHammer.


% TRRespass do not explain why they are able to bypass TRR
%TRRespass~\cite{frigo2020trrespass} automatically finds many-sided RowHammer
%access patterns that circumvent some of the current TRR implementations.
%However, the fuzzing-based approach that TRRespass implements has \textbf{two major
%limitations}. First, TRRespass finds effective RowHammer access patterns for
%\emph{only} 13 out of the 42 DRAM modules that the authors analyze. TRRespass
%fails to find any RowHammer access pattern that bypasses the TRR implementation
%of DRAM devices from one of the major three vendors. Second, TRRespass does
%\emph{not} provide sufficient insight on why specific access pattern cause
%RowHammer bit flips. Such insights are important to understand the weaknesses of
%the TRR implementations for not only developing more efficient RowHammer attacks but also
%addressing these weaknesses to provide better protection against RowHammer.


% Our goal is to understand TRR implementations to find access patterns that efficiently and effectively bypass TRR

% To this end, we propose a methodology to reverse engineer in-DRAM TRR and refresh
% The key idea is to use retention failures

%Leveraging the understanding of how a RowHammer mitigation mechanism works, we
%aim to explore access patterns that target the weaknesses of the mitigation
%mechanism to invalidate its protection.

%To this end, we propose a methodology to gain visibility into when a TRR
%mechanism performs victim row refresh and which victim rows it targets. 

%time to determine when the TRR mechanism refreshes the row by observing the retention
%time failures in the same row.


% Overview of the methodology

% The key
% idea of our methodology is to precisely profile the retention time of a row and use the
% row as a potential victim row by hammering the rows that are physically adjacent
% to the victim row at the halfway until the end of the victim's retention time. 





\vspace{1mm}
\noindent \textbf{\methodunformatted.} We develop \method{}, a \hhth{new and}
practical methodology that \hhf{uncovers} the inner workings of TRR mechanisms
in modern DRAM \hht{chips}. \hhth{To develop \method{}, we formulate} TRR as a
function that takes a number of DRAM accesses including \hhth{aggressor rows} as
input and refreshes a number of rows that are detected as victims. \hht{The goal
of} \method{} \hhth{is to enable the observation (i.e., uncovering) of} all
refreshes generated by TRR after \hhth{inducing a carefully crafted sequence of
DRAM accesses}. To make this possible, we make a key observation that retention
failures \hhf{that occur} on a DRAM row can be used as a side channel to detect
\hh{\emph{when} the row is} refreshed, due to \hht{either} TRR or \hh{periodic
refresh operations}. \hhth{We easily distinguish TRR-induced refreshes from
regular refreshes as the latter occur at fixed time intervals independently of
the access pattern.} 

We build two new tools, \rtplong{} \hhf{(\rtp{})} and \trranlong{}
\hhs{(\trran{})}, that make use of this \hhth{new} observation \hhth{to
construct \method{} and thus enable} a deep analysis of TRR. \hhf{The goal of
\rtp{} is to find a set of DRAM rows \hhf{that meet certain requirements as
needed by a \trran{} experiment} and identify the data retention times of these
rows. The goal of \trran{} is to use the \rtp{}-provided rows to determine when
a TRR mechanism refreshes a victim row by exactly distinguishing between TRR
refreshes and regular refreshes, and thus build an understanding of the
underlying TRR operation.}

\hht{\rtplong{} (\rtp{})} \hhth{profiles} \hht{the \hhth{data} retention time of
DRAM rows and passes to \trran{} a list of rows that satisfy two key
requirements}. First, a DRAM row should have a \emph{consistent} retention time
\hht{that does \emph{not}} vary over time based on effects such as Variable
Retention Time (VRT)~\hht{\cite{qureshi2015avatar, yaney1987meta,
liu2013experimental, restle1992dram}}. \hht{\rtp{} should not \hhf{supply to
\trran{}} a row with an inconsistent retention time since it would not be
possible for \trran{} to distinguish whether the row has been refreshed or it
simply retained its data correctly for longer than the profiled retention time.}
%
Second, \hhth{to enable observing how many and which DRAM rows TRR treats as
victim rows,} \hht{\rtp{} should provide \emph{multiple}} DRAM rows \hht{that}
have similar retention times and \hhf{that are} located at \hht{certain
\emph{configurable}} distances with respect to each other. \hhth{It is crucial
to find rows with similar retention times in order to observe whether or not TRR
can refresh multiple rows at the same time.} These two requirements enable
reliable and precise analysis \hhth{of TRR-induced refreshes} by \trran{}. 

\hhth{\hhs{\trranlong{} (\trran{})} discovers 1) access patterns that
\hhf{cause} the TRR mechanism to treat a certain row as an aggressor row and 2)
when a TRR-induced refresh targets a victim row.}
%
% \hh{At a high level, \trran{} detects a
% \hhf{TRR-induced refresh operation} \hhth{to an \rtp{}-provided row}  by
% \emph{not} observing a \hhth{bit flip (after not refreshing \hhf{the
% \rtp{}-provided row} row for its profiled retention time)} \hhth{on that row
% since retention failures are} expected on rows that TRR does \emph{not}
% refresh. \trran{} operates in three main steps.}
%
% \hhf{At a high level, \jk{\todo{How about:} \trran{} infers the occurrence of a
% TRR-induced refresh operation to an \rtp{}-provided row if that row does not
% contain any bit flips after the row's \rtp{}-profiled retention time (during
% which refreshes and accesses to the row are prevented). During the retention
% time period, only a TRR-induced refresh operation can refresh the
% \rtp{}-provided row and prevent the row from manifesting bit flips as a result
% of charge leakage.} 
%
\hhf{At a high level, \jk{\trran{} infers the occurrence of a TRR-induced
refresh operation to an \rtp{}-provided row {if the row does \emph{not} contain
any bit flips \hhf{after disabling regular refreshes and accesses to the row for
its \rtp{}-profiled retention time.} Only a TRR-induced refresh can prevent the
\rtp{}-provided row from experiencing bit flips} by refreshing the row before it
experiences a retention failure.} Thus, \trran{} attributes \emph{not} observing
a bit flip in an \rtp{}-provided row to TRR-induced refresh.}


\trran{} operates in three main steps. First, it initializes \hh{to known data
(e.g., all \emph{ones}) i) the \hht{\rtp{}-provided rows} and ii) the \hht{rows
\hhth{it selects} as aggressor rows in the experiment}}. Then, \trran{} lets the
\hht{\rtp{}-provided rows} leak their charge for half of their profiled
retention time. Second, \trran{} hammers (i.e., \hhf{repeatedly} activates and
precharges) the \hht{aggressor rows}. \hhf{After the hammers,} \trran{}
\hhf{issues} a small number of \hh{DRAM refresh commands (originally used for
only periodic refresh)} so \hhf{that} the \hhf{TRR-induced} row refresh can take
place.\footnote{\hhth{The current TRR implementations avoid changing the DDR
interface by piggybacking TRR-induced refreshes to regular refresh
commands~\cite{frigo2020trrespass, yauglikcci2021security}.}} \trran{} \jk{then}
waits for the \hhth{remaining} half of the profiled retention time.  \jk{If an
\rtp{}-provided row was not refreshed by TRR-induced refresh operations as a
result of the hammers issued by \trran{}, the \rtp{}-provided row would now have
not been refreshed for its full profiled retention time and will contain bit
flips.} 
% to \hhth{cause} the \hht{\rtp{}-provided rows to}
%\hhth{remain \hhf{not refreshed} for longer than their profiled retention time}
%\hhf{when the refresh commands in step two do not refresh these rows}. 
Third, \trran{} reads back the data stored in the \hht{\rtp{}-provided rows}
and checks for bit flips. \hhf{\emph{Observing no bit flips}} \hhth{in an
\rtp{}-provided row} indicates that \hhth{either a TRR-induced or regular
refresh, which \trran{} can easily distinguish \hhf{between} since the regular
refreshes happen periodically,} targeted the \hhth{same row} during step two.
In contrast, \emph{observing \hhth{bit flips}} indicates that the
\hhth{\rtp{}-provided row was} never refreshed. These three steps constitute
the core of the experiments that we conduct to understand different in-DRAM TRR
implementations.

% Case study 1: Reverse-engineering and Bypassing Samsung TRR
\vspace{1mm}
\noindent \textbf{Security analysis of TRR.} We use the \rtp{} and \trran{} on
\numTestedDIMMs{} DDR4 modules from the three major DRAM chip vendors (i.e.,
Micron, Samsung, SK Hynix). Our methodology \hhf{uncovers} important details of the
in-DRAM TRR designs of all vendors. We demonstrate the usefulness of these
insights \hhth{for} developing effective RowHammer attacks \hhth{on} DRAM
\hht{chips} from \hh{each vendor} by crafting specialized DRAM access patterns
that hammer \hht{a row} enough times to cause a RowHammer bit flip
\emph{without} alerting the TRR protection \hhth{mechanism} (i.e., \hhf{by}
redirecting \hhf{potential TRR} refreshes \emph{away from} the victim rows).
\hhth{In our evaluation, we find that all tested DRAM modules with different
manufacturing dates \hhf{(from 2016 to 2020)} are vulnerable to the new access
patterns we can craft via \method{}. Further, we find that \hhf{1) over
\vulnRowsMaxPct{}\% of the DRAM rows are vulnerable (i.e., have at least one bit
flip) to the new access patterns and 2) the new access patterns cause up to
\maxPerBankBitflips{} bit flips per DRAM bank.}} The large number of RowHammer
bit flips caused by our specialized \hhth{access} patterns has significant
implications for systems protected by \hhth{Error Correction Codes
(ECC)}~\cite{kang2014co,patel2020beer, patel2019understanding, patel2021harp}. Our analysis
shows that \hhf{the \method{}-discovered} access patterns can cause up to 7 bit
flips \hhf{at arbitrary locations} in one 8-byte dataword, suggesting that
typical ECC schemes capable of correcting one \hhth{error/symbol and detecting
two errors/symbols (e.g., SECDED ECC~\cite{micron2017whitepaper, oh2014a,
kwak2017a, kwon2017an, im2016im, son2015cidra, cha2017defect, jeong2020pair} and
Chipkill~\cite{dell1997white, nair2016xed, amd2009bkdg})} \hhf{\emph{cannot}}
provide sufficient protection against RowHammer \hhf{even in the presence of TRR
mechanisms}.


%To check whether system-level ECC can correct the bit flips that
%the new access pattern causes, we further analyze the number of bit flips in
%each cache line. We find that \ECCvulnCacheLinesPct{} of all cache lines with at
%least one bit flip have two or more bit flips, suggesting that ECC would not
%protect the system against RowHammer attacks that use this access pattern.

%Overall, our analysis shows that the new RowHammer access pattern causes bit flips in majority of the rows (i.e., an attacker can target almost any DRAM rows) and a significant number of cache lines has two or more bit flips, making ECC insufficient to cover these RowHammer bit flips.


% We expect researchers to adopt this tool to use in other current and future devices
\vspace{1mm}
\noindent \textbf{Contributions.} We expect that \method will help future
research on \hhf{both} evaluating the security of existing RowHammer protections and the
design of more secure \hhth{RowHammer mitigation} \hh{mechanisms}. In summary,
we make the following \hhth{major} contributions:

\squishlist

    \item We develop \method{}, a \hhf{new} methodology for reverse-engineering
    \hhth{Target Row Refresh (TRR)} and regular refresh \hhf{mechanisms}. 
    %\hh{We leverage the retention failures in
    % a DRAM row to gain visibility into when a TRR mechanism performs a targeted
    % refresh operation on the same row.}
    
    \item We use \method{} to \hhth{understand and uncover} the TRR
    implementations of \numTestedDIMMs{} DDR4 modules from the three \hhf{major
    DRAM} vendors. This evaluation shows that our \hhf{new} methodology is broadly
    applicable to any DRAM chip.

    \item Leveraging the TRR implementation details uncovered by \method{}, we
    craft specialized RowHammer access patterns that make \hhf{existing} TRR protections
    ineffective. 
    
    \item \hhth{Our specialized \hhf{\method{}-discovered} access patterns are
    significantly more effective than patterns from \hhth{the
    state-of-the-art}~\cite{frigo2020trrespass}: we show that our \hhs{new} RowHammer
    \hhth{access patterns cause} \hhf{1) bit flips \hhe{in \numTestedDIMMs{}} DDR4
    modules we comprehensively examine,} 2) bit flips in up to
    \vulnRowsMaxPct{}\% of the all rows in a DRAM bank, and 3) two and more (up
    to $7$) bit flips in a single 8-byte dataword, enabling practical RowHammer
    attacks in \hhth{systems that employ} ECC.}
        
\squishend


==> mainmatter/u-trr/2_background.tex <==
\section{Background}
\label{utrr_sec:background}

We provide background on DRAM and the RowHammer phenomenon that is required for
the reader to understand how \method{} can precisely uncover the behavior of an
in-DRAM RowHammer mitigation mechanism. For more detailed descriptions of DRAM
organization and operation, we refer the reader to many prior
works~\cite{chang2016understanding, chang2014improving, chang2016low,
chang2017understanding, hassan2019crow, hassan2016chargecache, kim2014flipping,
kim2012case, lee2015adaptive, lee2013tiered, lee2016simultaneous, lee2017design,
lee2015decoupled, liu2012raidr, liu2013experimental, seshadri2013rowclone,
seshadri2017ambit, seshadri2015gather, seshadri2020indram, zhang2014half,
kim2020revisiting, frigo2020trrespass, luo2020clr, yaglikci2021blockhammer,
wang2020figaro, cojocar2020are, patel2019understanding, bhati2015flexible,
zhang2016restore, kim2019d, kim2018dram, olgun2021quac, kim2015ramulator}.

\subsection{DRAM Organization} 

Fig.~\ref{utrr_fig:dram_organization} shows the typical organization of a modern DRAM
system. DRAM is organized into a hierarchical array of billions of DRAM cells,
each holding one bit of data. In modern systems, a CPU chip implements a set of
memory controllers, where each memory controller interfaces with a DRAM
\emph{channel} to perform read, write, and maintenance operations (e.g.,
refresh) via a dedicated I/O bus that is independent of other channels in the
system. A DRAM channel can host one or more \emph{DRAM modules}, where each
module consists of one or more \emph{DRAM ranks.} A rank is comprised of
multiple \emph{DRAM chips} that operate in lock step and ranks in the same
channel time-share the channel's I/O bus.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=.9\linewidth]{figures/dram_organization.pdf}
    \caption{Typical DRAM system organization.}
    \label{utrr_fig:dram_organization}
\end{figure}

A DRAM chip consists of multiple DRAM \emph{banks}, which share an internal
data/command bus.  Within a DRAM bank, DRAM cells are organized into multiple
(e.g., 128) dense two-dimensional arrays of DRAM cells called
\emph{subarrays}~\cite{kim2012case,chang2014improving,seshadri2013rowclone} and
corresponding peripheral circuitry for manipulating the data within the
subarray. A row of cells (i.e., DRAM \emph{row}) within a subarray share a wire
(i.e., \emph{wordline}), which is driven by a \emph{row decoder} to \emph{open}
(i.e., select) the row of cells to be read or written. A column of cells (i.e.,
DRAM \emph{column}) within a subarray share a wire (i.e., \emph{bitline}), which
is used to read and write to the cells with the help of a \emph{row buffer}
(consisting of \emph{sense amplifiers}). This hierarchical layout of DRAM cells
enables any data in the DRAM system to be accessed and updated using unique
rank, bank, row, and column addresses. 

\subsection{DRAM Operation} 

The memory controller interfaces with DRAM using a series of commands sent over
the I/O bus. To read or write data, the memory controller must first issue an
\emph{activate} (\cmdact{}) command to \emph{open} a row corresponding to the
provided memory address. When a row is activated, the data within the DRAM row
is copied into the row buffer of the subarray. The memory controller then issues
\emph{READ} (\cmdread{}) or \emph{WRITE} (\cmdwrite{}) commands to read or
update the data in the row buffer. Changes to the data in the row buffer
propagate to the DRAM cells in the opened row. When data from another row is
required, the memory controller must first issue a \emph{precharge}
(\cmdprech{}) command that \emph{closes} the open row and prepares the bank for
the activation of another row. 


\noindent\textbf{DRAM Refresh.} A DRAM cell stores a data value in the form of
charge in its capacitor (e.g., a charged cell can represent 0 or 1 and vice
versa). Since the capacitor naturally loses charge over time, the capacitor
charge must be actively and periodically \emph{refreshed} to prevent information
loss due to a data retention failure~\cite{patel2017reaper, jedec2014lpddr4,
jedec2008ddr3, liu2013experimental, khan2014efficacy, khan2017detecting,
khan2016parbor, liu2012raidr}. To enable such periodic refresh of all DRAM cells, the
memory controller must periodically issue a \emph{refresh} (\cmdrefresh{})
command (e.g., every \SI{7.8}{\micro\second}) to ensure that every DRAM cell is
refreshed once at a fixed \emph{refresh interval} (i.e., typically 32 or
\SI{64}{\milli\second})~\cite{jedec2014lpddr4, jedec2008ddr3,
liu2013experimental, liu2012raidr}.

\subsection{RowHammer} 

Modern DRAM chips suffer from disturbance errors that occur when a high number
of activations (within a refresh interval) to one DRAM row unintentionally
affects the values of cells in nearby rows~\cite{kim2014flipping}. This
phenomenon, popularly called \emph{RowHammer}~\cite{kim2014flipping,
mutlu2019rowhammer}, stems from electromagnetic interference between circuit
elements. RowHammer becomes exacerbated as manufacturing process technology node
size (and hence DRAM cell size) shrinks and circuit elements are placed closer
together~\cite{kim2020revisiting,mutlu2017rowhammer}. As demonstrated in prior
work~\cite{kim2014flipping, kim2020revisiting}, the RowHammer effect is
strongest between immediately physically-adjacent rows. RowHammer bit flips are
most likely to appear in neighboring rows physically adjacent to a
\emph{hammered row} that is activated many times (e.g., $139K$ in
DDR3~\cite{kim2014flipping}, $10K$ in DDR4~\cite{kim2020revisiting}, and $4.8K$
in LPDDR4~\cite{kim2020revisiting})\footnotemark[1]. A hammered row is also
called an \emph{aggressor row} and a nearby row that is affected by the hammered
row is called a \emph{victim row}, regardless of whether or not the victim row
actually experiences RowHammer bit flips.

\begin{figure}[!ht]
    \captionsetup[subfigure]{justification=centering, size=scriptsize}
    \centering
    \begin{subfigure}[b]{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/single_sided_rh.pdf}
    \end{subfigure}\quad
    \begin{subfigure}[b]{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/double_sided_rh.pdf}
    \end{subfigure}
    \caption{Typical Single-sided (SS) and Double-sided (DS) RowHammer access patterns.}
    \label{utrr_fig:rowhammer_access}
\end{figure}

To most effectively exploit the RowHammer phenomenon, attackers typically
perform $i$) single-sided RowHammer (i.e., repeatedly activate one aggressor row
that is physically adjacent to the victim row, as we show in
Fig.~\ref{utrr_fig:rowhammer_access}a)~\cite{kim2014flipping} or $ii$) double-sided
RowHammer (i.e., repeatedly activate in an alternating manner two aggressor rows
that are both physically adjacent to the victim row, as we show in
Fig.~\ref{utrr_fig:rowhammer_access}b)~\cite{seaborn2015exploiting, rh_project_zero}.
Prior works have shown that double-sided RowHammer leads to more bit flips and
does so more quickly than single-sided
RowHammer~\cite{kim2014flipping,kim2020revisiting, mutlu2019rowhammer,
seaborn2015exploiting, rh_project_zero}.

\subsection{RowHammer Mitigation Mechanisms}
\label{utrr_subsec:rh_mitigation}

To combat attacks that exploit the RowHammer phenomenon, various RowHammer
mitigation mechanisms have been proposed in
literature~\cite{yaglikci2021blockhammer, kim2014flipping, park2020graphene,
apple2015about, brasser2016can, konoth2018zebram, van2018guardion, aweke2016anvil,
lee2019twice, seyedzadeh2017cbt, son2017making, you2019mrloc,
greenfield2016throttling, yauglikcci2021security, kim2022mithril,
taouil2021lightroad, devaux2021method}.\footnotemark[2]
%
Yaglikci et al.~\cite{yaglikci2021blockhammer} classify these mitigation
mechanisms into four groups: $i$) increasing the refresh rate to reduce the
number of activations that can be performed within a refresh
interval~\cite{apple2015about, kim2014flipping}, $ii$) isolating sensitive data
from DRAM rows that an attacker can potentially hammer~\cite{brasser2016can,
konoth2018zebram, van2018guardion}, $iii$) keeping track of row activations and
refreshing potential victim rows~\cite{aweke2016anvil, kim2014flipping,
lee2019twice, park2020graphene, seyedzadeh2017cbt, son2017making,
you2019mrloc, yauglikcci2021security, kim2022mithril, taouil2021lightroad,
devaux2021method}, and $iv$) throttling row activations to limit the times a row
can be activated within a refresh interval~\cite{yaglikci2021blockhammer,
kim2014flipping, greenfield2016throttling}. Many of these research proposals
describe the details of their proposed mechanisms and discuss their security
guarantees~\cite{kim2014flipping, yaglikci2021blockhammer, park2020graphene}.


Unfortunately, DRAM vendors currently implement different \emph{proprietary}
in-DRAM RowHammer mitigation mechanisms, which they broadly refer to as Target
Row Refresh (TRR)~\cite{frigo2020trrespass,
cojocar2019exploiting,kim2020revisiting, micronddr4trr}. TRR detects a
potential aggressor row and refreshes its neighbor rows. The vendors have so far
not disclosed the implementation details of their TRR mechanisms, and thus the
security guarantees of such TRR mechanisms \emph{cannot} be properly and openly
evaluated. 

In fact, a recent work, TRRespass~\cite{frigo2020trrespass}, shows
that existing proprietary in-DRAM TRR mechanisms can be circumvented via
many-sided RowHammer attacks, which aim to overflow the internal tables that TRR
uses to detect aggressor rows. As such, it is critical to develop a rigorous
methodology to understand the weaknesses of TRR mechanisms and develop more
secure alternatives.

\textbf{Our goal} is to study in-DRAM TRR mechanisms so that we
can understand how they operate, assess their security, and enable fully-secure
DRAM against RowHammer.

==> mainmatter/u-trr/3_overview.tex <==
\section{Overview of U-TRR}
\label{utrr_sec:overview}

\method{} is a new methodology for gaining visibility into Target Row Refresh
(TRR) operations. It enables system designers and researchers to understand how
TRR detects an aggressor row, when it refreshes the victim rows of the aggressor
row, and how many potential victim rows it refreshes. \method{} enables users to
easily conduct experiments that uncover the inner workings of the TRR mechanism
in an off-the-shelf DRAM module.

Figure~\ref{utrr_fig:methodology_overview} illustrates the two components of \method{}:
\rtplong{} (\rtp{}) and \trranlong{} (\trran{}). \rtp{} finds a set of DRAM rows
that meet certain requirements as needed by \trran{} and identifies the data
retention times of these rows. \trran{} uses the \rtp{}-provided rows to
distinguish between TRR refreshes and regular refreshes, and thus builds an
understanding of the underlying TRR mechanism.

\begin{figure}[!h]
    \centering
    \includegraphics[width=.9\linewidth]{figures/utrr_overview.pdf}
    \caption{Overview of \method{}.}
    \label{utrr_fig:methodology_overview}
\end{figure}

\subsection{Overview of \rtplong{} (\rtp{})}

The goal of \rtp{} is to identify a list of useful DRAM rows and their retention
times, and provide this list to \trran{}. \rtp{} profiles the retention time of
a DRAM row by writing a data pattern (e.g., all
ones)~\cite{liu2012raidr,liu2013experimental} to the entire row and measuring the time
interval for which the row can correctly retain its data without being
refreshed.

A useful DRAM row must satisfy two key requirements. First, the retention time
of the row should be consistent and \emph{not} vary over time based on effects
such as Variable Retention Time (VRT)~\cite{kang2014co, khan2014efficacy,
liu2013experimental, mori2005origin, qureshi2015avatar, restle1992dram,
yaney1987meta}. A consistent retention time is essential for \trran{} to
accurately infer whether or not a row has been refreshed after a specific time
interval, based on whether or not the row contains retention failures. \rtp{}
validates the retention time of a row one thousand times to ensure its
consistency over time.

Second, to observe exactly which DRAM rows the TRR mechanism treats as victim
rows for each aggressor row it detects, \rtp{} should provide \emph{multiple}
DRAM rows that have the \emph{same} retention times and that are located at
certain \emph{configurable} distances with respect to each other (we call this a
\emph{row group}). It is crucial to find rows with the same retention times in
order to observe whether or not TRR can refresh \emph{multiple} rows at the same
time. Enforcing a particular distance between rows is useful when the user wants
to specify an aggressor row at a specific distance from the \rtp{}-provided
rows. These two requirements enable reliable and precise analysis of TRR-induced
refreshes by \trran{}.

As shown in Figure~\ref{utrr_fig:methodology_overview}, the number of row groups (i.e.,
row group count) and the relative distances of the rows within the group (i.e.,
row group layout) is specified in the \emph{profiling configuration}. \method{}
user also specifies a certain DRAM bank and row range within the bank for the
\rtp{} to search for the desired row groups. We discuss the operation and
capabilities of \rtp{} in greater detail in \cref{utrr_sec:ret_profiling}.


\subsection{Overview of \trranlong{} (\trran{})}
\label{utrr_subsec:trran_overview}

The goal of \trran{} is to use \rtp-provided rows to determine when a TRR
mechanism refreshes a victim row by exactly distinguishing between TRR refreshes
and regular refreshes, and thus build an understanding of the underlying TRR
operation. \trran{} runs a RowHammer attack and monitors retention failures in
\rtp{}-provided rows to determine \emph{when} TRR refreshes any of these rows.
As Figure~\ref{utrr_fig:methodology_overview} shows, \trran{} operates based on an
\emph{experiment configuration}, which includes several parameters we discuss in
\cref{utrr_subsec:trr_operation}. Figure~\ref{utrr_fig:general_trr_detection_approach}
shows the three steps a \trran{} experiment generally follows:
\begin{enumerate} 
    \item \trran{} uses \rtp{}-provided rows as victim rows and
        initializes~\circled{1} them by writing into them the same data pattern
        that is used during retention profiling with \rtp{}. Since the RowHammer
        vulnerability greatly depends on the data values stored in an aggressor
        row~\cite{kim2020revisiting,kim2014flipping}, \trran{} also initializes
        aggressor rows to the data values that the user specifies in the
        experiment configuration. \trran{} waits for half of the victim rows'
        retention time ($\frac{T}{2}$) without performing any refreshes or
        accesses.

    \item \trran{} hammers~\circled{2} the aggressor rows and issues
        \cmdrefresh{}~\circled{3} commands based on the experiment
        configuration.

    \item After again waiting for the half of the victim rows' retention time
        ($\frac{T}{2}$), excluding the time spent on hammering and refresh
        during step (2), \trran{} reads the victim rows and
        compares~\circled{4} the data stored in them against the initial data
        value pattern written to them in step (1). A victim row with no bit
        flips indicates that either a TRR-induced or a regular refresh operation
        targeted the victim row while serving the \cmdrefresh{} commands in step
        (2). \trran{} easily distinguishes between a TRR-induced and a regular
        refresh as the latter refreshes a row periodically (e.g., once in every
        $8K$ \cmdrefresh{} commands). The user can then examine the TRR-induced
        refresh patterns to gain insight into the underlying TRR implementation.
\end{enumerate}

\begin{figure}[!h]
    \centering
    \includegraphics[width=.85\linewidth]{figures/general_trranalyzer_approach.pdf}
    \caption{General approach for detecting a TRR-induced refresh using
    \trran{}.}
    \label{utrr_fig:general_trr_detection_approach}
\end{figure}

\trran{} offers flexibility in experiments via parameters in the profiling and
experiment configurations, which enable analyzing different TRR implementations
with low effort. \cref{utrr_sec:analyzing_refs} provides details.

\subsection{Required Experimental Setup for \method{}}
\label{utrr_subsec:softmc}

Both the \rtp{} and \trran{} tools require a way to directly interface with a
DRAM module at a DDR-command level. This is because the tools need to accurately
control when an individual DDR command (e.g., \cmdact{}, \cmdrefresh{}) is
issued to the DRAM module. However, existing systems based on commodity CPUs can
access DRAM \emph{only} using load/store instructions. Therefore, we implement
\rtp{} and \trran{} using SoftMC~\cite{hassan2017softmc,softmcsource}, an
FPGA-based DRAM testing infrastructure that provides precise control on the DDR
commands issued to a DRAM module. We modify SoftMC to support testing DDR4
modules, as also done in~\cite{kim2020revisiting,olgun2021quac, orosa2021deeper,
frigo2020trrespass}. Figure~\ref{utrr_fig:utrr_photo} shows our experimental
SoftMC setup. Table~\ref{utrr_table:trr_summary} provides a list of the
\numTestedDIMMs{} DDR4 DRAM modules we analyze in this \hhm{chapter}.

\begin{figure}[!h]
    \centering
    \includegraphics[width=.8\linewidth]{figures/softmc_photo.pdf}
    \caption{DDR4 SO-DIMM SoftMC~\cite{hassan2017softmc} experimental setup.}
    \label{utrr_fig:utrr_photo}
\end{figure}

==> mainmatter/u-trr/8_related_work.tex <==
\section{Related Work}
\label{utrr_sec:related_work}


% explain how rh spreads starting from kim2014flipping
Kim et al.~\cite{kim2014flipping} are the first to introduce and analyze the
RowHammer phenomenon. Numerous later works develop RowHammer attacks to
compromise various systems in various ways~\cite{cojocar2019exploiting,
gruss2018another, gruss2016rowhammer, lipp2018nethammer, qiao2016new,
razavi2016flip, seaborn2015exploiting, tatar2018defeating, veen2016drammer,
xiao2016one, frigo2020trrespass, ji2019pinpoint, kwong2020rambleed,
mutlu2017rowhammer, van2018guardion, kim2020revisiting, deridder2021smash,
mutlu2019rowhammer, pessl2016drama, bosman2016dedup, bhattacharya2016curious,
jang2017sgx, aga2017good, frigo2018grand, hong2019terminal, cojocar2020are,
weissman2020jackhammer, zhang2020pthammer, rowhammergithub, yao2020deephammer}
and analyze RowHammer further~\cite{cojocar2020are, cojocar2019exploiting,
gruss2018another, kim2020revisiting, qiao2016new, tatar2018defeating,
yang2019trap, walker2021dram, orosa2021deeper, google2021halfdouble}. To our
knowledge, this is the first work to 1) propose an experimental methodology to
understand the inner workings of commonly-implemented in-DRAM RowHammer
protection (i.e., TRR) mechanisms and 2) use this understanding to create custom
access patterns that circumvent the TRR mechanisms of modern DDR4 DRAM chips.


% discussion on TRRespass
% \vspace{1mm}
\noindent \textbf{In-DRAM TRR.} We already provided extensive descriptions of
TRR and TRRespass in \cref{bg:subsec:rowhammer}, \cref{utrr_sec:motivation}, and
\cref{utrr_sec:insights}. TRRespass~\cite{frigo2020trrespass} is the most relevant
prior work to ours in understanding and circumventing TRR mechanisms, yet it is
not effective enough. While TRRespass can incur RowHammer bit flips in 13 of 42
DDR4 modules (and 5 of 13 LPDDR4 modules), TRRespass does not uncover many
implementation details of the TRR mechanisms, which are important to circumvent
TRR mechanisms. For example, in 29 out of 42 DDR4 modules (and 8 out of 13
LPDDR4 modules), TRRespass fails to find an access pattern that can circumvent
TRR. In contrast, our new \method{} methodology can be used to understand
different aspects of a TRR mechanism in great detail and use this understanding
to generate specific RowHammer access patterns that effectively incur a large
number of bit flips (as we show on \numTestedDIMMs{} real DRAM modules).

% give hw based mitigation examples
% \vspace{1mm}
\noindent \textbf{System-level RowHammer Mitigation Techniques.} A number of
studies propose system-level RowHammer mitigation
techniques~\cite{yaglikci2021blockhammer, kim2014flipping, park2020graphene,
apple2015about, brasser2016can, konoth2018zebram, van2018guardion,
aweke2016anvil, lee2019twice, seyedzadeh2017cbt, son2017making, you2019mrloc,
greenfield2016throttling, yauglikcci2021security, kim2022mithril,
taouil2021lightroad, devaux2021method, woo2023scalable,
saileshwar2022randomized}. Recent works~\cite{frigo2018grand, gruss2018another,
yaglikci2021blockhammer, kim2020revisiting} show that some of these mechanisms
are insecure, inefficient, or do not scale well in chips with higher
vulnerability to RowHammer. We believe the fundamental principles of \method{}
can be useful for improving the security of these works as well as potentially
combining them with in-DRAM TRR. We leave examining such directions to future
work.

==> mainmatter/u-trr/9_conclusion.tex <==
\section{Summary}
\label{utrr_sec:conclusion}

We propose \method{}, a novel experimental methodology for reverse-engineering
the main RowHammer mitigation mechanism, Target Row Refresh (TRR), implemented
in modern DRAM chips. Using \method{}, we 1) provide insights into the inner
workings of existing proprietary and undocumented TRR mechanisms and 2) develop
custom DRAM access patterns to efficiently circumvent TRR in \numTestedDIMMs{}
DDR4 DRAM modules from three major vendors. We conclude that TRR does \emph{not}
provide security against RowHammer and can be easily circumvented using the new
understanding provided by \method{}. We believe and hope that \method{} will
facilitate future research by enabling rigorous and open analysis of RowHammer
mitigation mechanisms, leading to the development of both new RowHammer attacks
and more secure RowHammer protection mechanisms. \hhmiv{We open source our U-TRR
methodology and make it freely available for further research and
development~\cite{utrrsource}.}

==> mainmatter/u-trr/motivation_and_goal.tex <==
\section{Motivation and Goal}
\label{utrr_sec:motivation}

DRAM technology scaling leads to increasingly important DRAM reliability
problems as DRAM cells get smaller and the distance between the cell reduce. Kim
et al.~\cite{kim2014flipping} report that most DRAM chips manufactured since
2010 are susceptible to disturbance errors that are popularly referred to as
RowHammer. Recent works~\cite{yang2019trap, walker2021dram, kim2014flipping,
mutlu2019rowhammer, ryu2017overcoming, park2016experiments, yang2016suppression,
yang2017scanning, gautam2019row, jiang2021quantifying} explain the circuit-level
charge leakage mechanisms that lead to the RowHammer vulnerability. A security
attack exploits the RowHammer vulnerability by hammering (i.e., repeatedly
activating and precharging) an \emph{aggressor} row many times (e.g., $139K$ in
DDR3~\cite{kim2014flipping}, $10K$ in DDR4~\cite{kim2020revisiting}, and $4.8K$
in LPDDR4~\cite{kim2020revisiting})\footnote{For DDR3 chips,
\cite{kim2014flipping} reports the minimum number of row activations on a
\emph{single} aggressor row (i.e., single-sided RowHammer) to cause a RowHammer
bit flip. For DDR4 and LPDDR4 chips, \cite{kim2020revisiting} reports the
minimum number of row activations to \emph{each of the two} immediately-adjacent
aggressor rows (i.e., double-sided RowHammer).} to cause bit flips in the cells
of the \emph{victim} rows that are physically adjacent to the hammered row.
Since the discovery of RowHammer, researchers have proposed many techniques that
take advantage of the RowHammer vulnerability to compromise operating
systems~\cite{seaborn2015exploiting, van2018guardion, veen2016drammer,
gruss2016rowhammer, cojocar2019exploiting, qiao2016new, kwong2020rambleed,
pessl2016drama, bhattacharya2016curious, jang2017sgx, zhang2020pthammer,
cojocar2020are, weissman2020jackhammer, ji2019pinpoint}, web
browsers~\cite{gruss2018another, bosman2016dedup, frigo2020trrespass,
deridder2021smash, frigo2018grand}, cloud virtual machines~\cite{razavi2016flip,
xiao2016one}, remote servers~\cite{tatar2018defeating, lipp2018nethammer}, and
deep neural networks~\cite{yao2020deephammer, hong2019terminal}.\footnote{A
review of many RowHammer attacks and defenses is provided
in~\cite{mutlu2019rowhammer}.} Thus, RowHammer is a clear major threat to system
security.

To prevent RowHammer, DRAM vendors equip their DRAM chips with a
\emph{mitigation mechanism} known as Target Row Refresh
(TRR)~\cite{frigo2020trrespass, cojocar2019exploiting,kim2020revisiting,
micronddr4trr}. The main idea of TRR is to detect an aggressor row (i.e., a row
that is being rapidly activated) and refresh its victim rows (i.e., neighboring
rows that are physically adjacent to the aggressor row). TRR refreshes the
victim rows separately from the \emph{regular} refresh operations~\cite{liu2012raidr,
venkatesan2006retention, liu2013experimental, cui2014dtail, bhati2015flexible}
that must periodically (e.g., once every \SI{64}{\milli\second}) refresh each
DRAM row in the entire DRAM chip. Some of the major DRAM vendors advertise
\emph{RowHammer-free} DDR4 DRAM chips~\cite{lee2014green, micronddr4,
frigo2020trrespass}. However, none of the DRAM vendors have so far disclosed the
implementation details let alone proved the protection guarantees of their TRR
mechanisms. It is long understood that security cannot be achieved only through
obscurity~\cite{scarfone2008guide, anderson2020security, saltzer1975protection}.
Yet, such is the current state of practice when it comes to DRAM.

The recent TRRespass work~\cite{frigo2020trrespass} shows that in certain DRAM
chips, the TRR mechanism keeps track of only a few aggressor rows. Hence, an
access pattern that hammers many aggressor rows can circumvent the TRR
protection and induce RowHammer bit flips. While TRRespass already demonstrates
the flaws of certain TRR implementations, it does \emph{not} propose a
methodology for \emph{discovering} these flaws. According
to~\cite{frigo2020trrespass}, simply increasing the number of aggressor rows is
\emph{not} sufficient to induce bit flips on 29 out of 42 of the DDR4 modules
that were tested by~\cite{frigo2020trrespass}. However, it is unclear whether
such DDR4 chips are \emph{fully} secure due to the lack of insight into the
detailed operation of TRR in these chips. Thus, we need new methods for
identifying whether or not DRAM chips are fully secure against RowHammer.

To this end, \textbf{our goal} is to uncover the inner workings of TRR
mechanisms in modern DRAM chips and assess their security guarantees. To achieve
this goal, we develop \method{}, a new and practical methodology for
understanding the operation of an in-DRAM TRR mechanism. In \method{}, we
formulate TRR as a function that takes a number of DRAM accesses including
aggressor rows as input and refreshes a number of rows that are detected as
victims. \method{} is based on the key observation that retention failures that
occur on a DRAM row can be used as a side channel to detect \emph{when} the row
is refreshed, due to either TRR or periodic refresh operations. We easily
distinguish TRR-induced refreshes from regular refreshes as the latter occur at
fixed time intervals independently of the access pattern.

We use \method{} to analyze \numTestedDIMMs{} DDR4 modules from the three major
DRAM chip vendors (i.e., Micron, Samsung, SK Hynix). Our methodology uncovers
important details of the in-DRAM TRR designs of all vendors. We demonstrate the
usefulness of these insights for developing effective RowHammer attacks on DRAM
chips from each vendor by crafting specialized DRAM access patterns that hammer
a row enough times to cause a RowHammer bit flip \emph{without} alerting the TRR
protection mechanism (i.e., by redirecting potential TRR refreshes \emph{away
from} the victim rows).

==> mainmatter/u-trr/tables/tested_modules.tex <==
\begin{table}[!ht]
    
    \centering
    % \begin{yellowb}
    \caption{List of the analyzed DDR4 SODIMMs.}
    \label{table:tested_modules}

    \begin{threeparttable}
        \renewcommand{\arraystretch}{0.7}
        \resizebox{\linewidth}{!}{

            \begin{scriptsize}
                \begin{tabular}{ l l c c c c}
                    \toprule

                    \mr{2.5}{\emph{Module}} & \mr{2.5}{\emph{\makecell{Date\\(yy-ww)}}}  & \mr{2.5}{\emph{\makecell{Size\\(GB)}}} & \multicolumn{3}{c}{\emph{Organization}}\\

                    \cmidrule(lr){4-6}

                    \multicolumn{3}{c}{} & \emph{Ranks} & \emph{Banks} & \emph{Pins} \\

                    \midrule

                    %'sam15' : 'A0', 'sam22' : 'A1', 'gr00' : 'A2', 'sp00' : 'A3', 'sam11' : 'A4', 'sam12' : 'A5', 'sam14' : 'A6', 'sam10' : 'A7',  

                    \stripe
                    % \rowcolor[]{1}{white}{cyan}
                    A[0, 4-7] & 19-36 & 4 & 1 & 16 & x8 \\
                    A[1] & 19-45 & 4 & 1 & 16 & x16 \\
                    A[2] & 20-07 & 8 & 1 & 16 & x8 \\
                    A[3] & 19-50 & 8 & 1 & 16 & x8 \\
                    
                    % \stripe
                    
                    %'hytt05' : 'B0', 'hytt00' : 'B1', 'hytt01' : 'B2', 'hytt04' : 'B3', 'tf00' : 'B4', 'tf01' : 'B5', 'tf03' : 'B6', 'tim4' : 'B7',

                    \cmidrule(lr){1-6}
                    % \stripe
                    B[0-2] & 16-48 & 4 & 1 & 16 & x8 \\
                    B[3] & 19-06 & 16 & 2 & 16 & x8 \\
                    B[4-6] & 20-17 & 8 & 1 & 16 & x8 \\
                    B[7] & 18-22 & 4 & 1 & 16 & x8 \\

                    % 'at00' : 'C0', 'at01' : 'C1', 'cru0' : 'C2', 'cru2' : 'C3', 'micr00' : 'C4', 'micr02' : 'C5', 'miki00': 'C6', 'miki02' : 'C7',
                    \cmidrule(lr){1-6}
                    C[0-1] & 20-31 & 4 & 1 & 16 & x16 \\
                    C[2-5] & 16-48 & 4 & 1 & 16 & x8 \\
                    C[6-7] & 17-12 & 4 & 1 & 16 & x8 \\

                    \bottomrule
                \end{tabular}
            \end{scriptsize}
        }

    \end{threeparttable}

    % \end{yellowb}
\end{table}

==> mainmatter/u-trr/vars.tex <==

\newcommand{\methodunformatted}{U-TRR\xspace}
\newcommand{\method}{\texttt{\methodunformatted{}}\xspace}

\newcommand{\rtplong}{\emph{{Row Scout}}\xspace}
\newcommand{\rtp}{\emph{{RS}}\xspace}
\newcommand{\trranlong}{\emph{{TRR Analyzer}}\xspace}
\newcommand{\trran}{\emph{{\mbox{TRR-A}}}\xspace}

\newtheorem{obsA}{\textbf{Vendor A | Observation}}
\newtheorem{obsB}{\textbf{Vendor B | Observation}}
\newtheorem{obsC}{\textbf{Vendor C | Observation}}

\newtheorem{req}{Requirement}

\newcommand{\numTestedDIMMs}{45} % the total number of tested modules (all vendors)
\newcommand{\numTestedDIMMsFromA}{15} % the total number of tested modules from vendor A
\newcommand{\numTestedDIMMsFromB}{15} % the total number of tested modules from vendor A
\newcommand{\numTestedDIMMsFromC}{15} % the total number of tested modules from vendor A
\newcommand{\vulnRowsAveragePct}{X} % the percentage of rows with bitflips w.r.t. all rows in a bank
\newcommand{\vulnRowsMaxPct}{99.9} % the percentage of rows with bitflips w.r.t. all rows in a bank
\newcommand{\ECCvulnCacheLinesPct}{X} % the percentage of cache lines with 2 or more bitflips compared to number of cache lines with at least one bitflip
\newcommand{\maxPerBankBitflips}{9.4 million} % the max number of bitflips in a single DRAM bank
